A Spark Optimizer for Adaptive, Fine-Grained Parameter Tuning

As Spark becomes a common big data analytics platform, its growing complexity makes automatic tuning of numerous parameters critical for performance. Our work on Spark parameter tuning is particularly motivated by two recent trends: Spark's Adaptive Query Execution (AQE) based on runtime statistics, and the increasingly popular Spark cloud deployments that make cost-performance reasoning crucial for the end user. This paper presents our design of a Spark optimizer that controls all tunable parameters of each query in the new AQE architecture to explore its performance benefits and, at the same time, casts the tuning problem in the theoretically sound multi-objective optimization (MOO) setting to better adapt to user cost-performance preferences. To this end, we propose a novel hybrid compile-time/runtime approach to multi-granularity tuning of diverse, correlated Spark parameters, as well as a suite of modeling and optimization techniques to solve the tuning problem in the MOO setting while meeting the stringent time constraint of 1-2 seconds for cloud use. Evaluation results using TPC-H and TPC-DS benchmarks demonstrate the superior performance of our approach: (i) When prioritizing latency, it achieves 63% and 65% reduction for TPC-H and TPC-DS, respectively, under an average solving time of 0.7-0.8 sec, outperforming the most competitive MOO method that reduces only 18-25% latency with 2.6-15 sec solving time. (ii) When shifting preferences between latency and cost, our approach dominates the solutions of alternative methods, exhibiting superior adaptability to varying preferences.

==> Qi_compile_time_opt/overview.tex <==
% SortMergeJoin types of PQP and Why
% two options
% option 1: LQP model (ICDE work)
% option 2: LQP-sub model (current algorithm)


%general problem statement
%special case: reduced problem statement


% 1. short intro:
In this section, we present the compile-time optimization approach that finds the optimal configuration $\thetabm_c^*$ of the context parameters to construct an ideal Spark context for query execution. 
Our approach does so by exploring the correlation of $\thetabm_c$ with the $\bm{\theta_p}$ and $\bm{\theta_s}$ parameters for different subqueries, under the modeling constraints that the non-decision variables for cardinality estimates are based on Spark's cost-based optimizer. %data distributions are assumed to be uniform across partitions, and resource contention is not captured. 
Nevertheless, even under these modeling constraints, capturing the correlation between these three categories of parameters allows us to find a better Spark context for query execution, \todo{as we will demonstrate in our experimental study}. 

In addition, this process also determines the $\bm{\theta_p}$ and $\bm{\theta_s}$ parameters for the scan-based query stages, which do not have any dependencies on other query stages and are not covered by AQE at runtime. \yanlei{Do we use correct statistics for these scan-based query stages?}

%$\bm{\theta_p}$ and $\bm{\theta_s}$ are correlated, with $\bm{\theta_s}$ not influencing the scan-based QSs and being updated for following QSs during runtime. Consequently, we omit the optimization of $\bm{\theta_s}$ during compile-time optimization. \yanlei{Don't understand}


%During compile-time, our goal is to (a) configure the initial $\thetabm_p$ for the scan-based query stages, which do not have any dependencies on other stages and are not covered by AQE at runtime, and (b) by leveraging the correlation among all categories of parameters, find the optimal $\thetabm_c^*$ to construct an ideal Spark context for query execution. %$\Thetabms$
%Our compile-time optimization uses the cardinality estimates by Spark's default cost-based optimizer (setting the cardinality estimate variable as $\alpha=\alpha_{cbo}$), assuming a uniform data distribution across partitions (setting the data distribution variable as $\beta = \vec{0}$), and zero resource contention (the resource contention variable $\gamma = \vec{0}$). 


%\input{Qi_compile_time_opt/problem_statement_and_our_approach.tex}

\input{Qi_compile_time_opt/div_and_conq_moo.tex}

\input{Qi_compile_time_opt/LQP_tuning.tex}

\input{Qi_compile_time_opt/dag_opt.tex}


% challenges of compile-time optimization
%\minip{Technical issue: correlated $\bm{\theta_c}$, $\bm{\theta_p}$ and $\bm{\theta_s}$} Spark forces the fixing of context settings, including resources, at the beginning, and $\bm{\theta_c}$ is shared among all LQP-subtrees. This requires compile-time optimization to provide optimal $\bm{\theta_c}$ configurations before query execution.

%The effect of $\bm{\theta_p}$ extends to both the scan-based QSs determined at query compilation and the following QSs generated during runtime. Compile-time optimization is necessary to provide optimal $\bm{\theta_p}$ configurations for scan-based QSs.

%$\bm{\theta_c}$ and $\bm{\theta_p}$ are correlated during compile-time optimization. However, it is non-trivial to optimize $\bm{\theta_c}$ and $\bm{\theta_p}$  jointly by considering multiple objectives as they are under multi-granularity control. We proposed an algorithm to solve this issue. 

%$\bm{\theta_p}$ and $\bm{\theta_s}$ are correlated, with $\bm{\theta_s}$ not influencing the scan-based QSs and being updated for following QSs during runtime. Consequently, we omit the optimization of $\bm{\theta_s}$ during compile-time optimization.


% why fixing s4 in the \theta_p
% \texttt{SortMergeJoin} is more complex than \texttt{BroadcastHashJoin}

\subsection{Implementation Details}
$\bm{\theta_p}$ affects the choices for join types of the PQP from LQP at both compile time and runtime in Spark. 
It is recognized that employing a \texttt{BroadcastHashJoin} in Spark can yield savings in CPU and IO costs compared to a \texttt{SortMergeJoin}, specifically when one side of the join relation is sufficiently small to be broadcasted. However, it is noteworthy that Spark's support for transitioning from a \texttt{SortMergeJoin} to a \texttt{BroadcastHashJoin} occurs exclusively when there are updates to the parameters $\bm{\theta_p}$ during runtime. Conversely, the system does not allow a change from a \texttt{BroadcastHashJoin} to a \texttt{SortMergeJoin}. More precisely, if the input size of a join operator is overestimated at compile time (i.e., greater than the actual input size), Spark generates a Physical Query Plan (PQP) with a \texttt{SortMergeJoin}. Subsequently, it dynamically switches back to a \texttt{BroadcastHashJoin} at runtime, utilizing the accurate input size to achieve improved performance. Conversely, if the input size is underestimated at compile time (i.e., less than the actual input size), Spark generates a PQP with a \texttt{BroadcastHashJoin}, and it cannot dynamically switch to a \texttt{SortMergeJoin} at runtime, even if a \texttt{SortMergeJoin} would lead to superior performance.

This observation underscores that the choices made for join types in the PQP at compile time have a discernible impact on performance during runtime. To ensure that runtime optimization achieves superior performance, we strive for a PQP with \texttt{SortMergeJoin} types established at compile time. Consequently, the compile-time optimization tends to overestimate resources for runtime optimization, potentially leading to a reduction in latency.


\cut{
% original text
It is known that \texttt{BroadcastHashJoin} saves CPU and IO cost compared to \texttt{SortMergeJoin} if one side of the join relation is smaller enough to be broadcasted.
However, Spark only supports transition from \texttt{SortMergeJoin} to \texttt{BroadcastHashJoin} when $\bm{\theta_p}$ updates at runtime, and cannot change from \texttt{BroadcastHashJoin} to \texttt{SortMergeJoin}. More specifically, if the input size of a join operator is overestimated (i.e. greater than the real input size) at compile time, Spark generates a PQP with \texttt{SortMergeJoin} and it will change back to \texttt{BroadcastHashJoin} with the real input size at runtime to achieve better performance. 
If the input size is underestimated (i.e. lower than the real input size) at compile time, Spark generates a PQP with \texttt{BroadcastHashJoin} and it cannot change to \texttt{SortMergeJoin} at runtime even if \texttt{SortMergeJoin} results in better performance. 

It indicates that the choices for join types of the PQP at compile time affect the performance at runtime. To guarantee the runtime optimization achieves better performance, we aim at a PQP with \texttt{SortMergeJoin} type produced at compile time. Then the compile-time optimization will overestimate resources for the runtime optimization, which could further reduce the latency.
}

==> Qi_compile_time_opt/problem_statement_and_our_approach.tex <==
\subsection{Overview of our Approach}
\label{subsec:compile_time_moo}

We assume that the input size $\alpha$ and data distribution $\beta$ are accurately known at compile time, and that there is no runtime contention $\gamma$. For the sake of simplification, we omit the non-decision variables $\alpha$, $\beta$, and $\gamma$ in the following general multi-objective optimization (MOO) problem definition during compile-time.

%\minip{\underline{Option 1}}: 
%We define a general Query-level MOO problem by employing the LQP model as follows. The parameters are under coarse-grained control, where $\bm{\theta_{p}}$ is uniformly set for all the LQP-subtrees.
%
%{\definition{\textbf{Query-level MOO with Coarse-grained control.}
%		\begin{eqnarray}
%		\label{eq:general_query_moo_def}
%		\arg \min_{\bm{\theta}} F(\bm{\theta})=& {\left[
%			\begin{array}{l}
%			F_1(\bm{\theta}) = \Phi_1(LQP, \bm{\theta_c},\bm{\theta_{p}}) \\ 
%			...\\
%			F_k(\bm{\theta}) = \Phi_k(LQP, \bm{\theta_c},\bm{\theta_{p}})
%			\end{array}
%			\right]} \\
%		\nonumber s.t. &
%		\bm{\theta_c} \in  \mathbb{R}^{d_c} \in \Sigma_c \quad \bm{\theta_{p}} \in  \mathbb{R}^{d_p} \in \Sigma_p\\
%		\end{eqnarray}
%}}

%\noindent{ 
%where we denote $\bm{\theta} = [\bm{\theta_c}, \bm{\theta_{p}}]$, which represents configurations for the entire query. Here, $\bm{\theta_{p}}$ is uniformly set for all the LQP-subtrees, and $\Phi_j$ denotes the LQP model for the $j$-th objective, where $j = 1, \ldots, k$.
%}
%
%The optimization problem in Option 1 is a general multi-objective optimization (MOO) problem, which can be solved by any existing MOO method, including the Progressive Frontier approach introduced in our prior work \cite{spark-moo-icde21}. However, it does not provide support for fine-grained control over $\bm{\theta_{p}}$, and as a result, it cannot guarantee the discovery of true Pareto optimal solutions.


%\minip{\underline{Option 2}}: we define a general Query-level MOO problem by applying LQP-sub model as following. It involves fine-tuning $\bm{\theta_{p}}$ for each LQP-subtree.
%
%{\definition{\textbf{General Query-level MOO with Fine-grained control.}
%		\begin{eqnarray}
%		\label{eq:general_query_moo_def}
%		\arg \min_{\bm{\theta}} F(\bm{\theta})=& {\left[
%			\begin{array}{l}
%			F_1(\bm{\theta}) = \Psi_1(LQP, \bm{\theta_c},\bm{\theta_{p1}},...,\bm{\theta_{pm}}) \\ 
%			...\\
%			F_k(\bm{\theta}) = \Psi_k(LQP, \bm{\theta_c},\bm{\theta_{p1}},...,\bm{\theta_{pm}})
%			\end{array}
%			\right]} \\
%		\nonumber s.t. &
%		\bm{\theta_c} \in  \mathbb{R}^{d_c} \in \Sigma_c \quad \bm{\theta_{pi}} \in  \mathbb{R}^{d_p} \in \Sigma_p, \quad i = 1,..., m\\
%		\end{eqnarray}
%}}

%\noindent{ 
%Where we denote $\bm{\theta} = [\bm{\theta_c}, \bm{\theta_{p1}}, \ldots, \bm{\theta_{pm}}]$, representing the configuration for the entire query. Here, $m$ is the number of LQP-subtrees, and $\Psi_j$ is the query-level predictive model for the $j$-th objective. In other words, $\Psi_j$ is a query-level model composed of LQP-sub models, where $j=1, \ldots, k$.
%}
%
%The optimization problem in Option 2 provides fine-grained control over $\bm{\theta_{p}}$. The total parameter space is $d_c + m \cdot d_p$. However, it suffers from the high-dimensionality issue, especially when $m$ is large.


The optimization problem in Option 2 provides fine-grained control over $\bm{\theta_{p}}$. The total parameter space is $d_c + m \cdot d_p$. However, it suffers from the high-dimensionality issue, especially when $m$ is large.


\minip{Our Approach:}
To address the high-dimensionality issue of the parameter space, we propose an algorithm named \textit{Divide-and-Conquer MOO}. This algorithm follows a divide-and-conquer framework, where the problem is defined as follows:


{\definition{\textbf{Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:div_query_moo_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})={\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Lambda(\phi_1(LQP_1, \bm{\theta_c},\bm{\theta_{p1}}),...,\\\phi_1(LQP_m, \bm{\theta_c},\bm{\theta_{pm}})) \\ 
			...\\
			F_k(\bm{\theta}) = \Lambda(\phi_k(LQP_1, \bm{\theta_c},\bm{\theta_{p1}}),...,\\\phi_k(LQP_m, \bm{\theta_c},\bm{\theta_{pm}}))
			\end{array}
			\right]} \\
		\nonumber s.t. & \bm{\theta_c} \in  \mathbb{R}^{d_c} \in \Sigma_c \quad \bm{\theta_{pi}} \in  \mathbb{R}^{d_p} \in \Sigma_p, \quad i = 1,..., m\\
%		& \bm{\theta_{si}} \in  \mathbb{R}^{d_s} \in \Sigma_s, \quad i = 1,..., m\\		
		\end{eqnarray}
}}

\noindent{
Where we denote $\bm{\theta_i} = [\bm{\theta_c},\bm{\theta_{pi}}]$, representing configurations for a LQP-subtree $LQP_i$ within a query, with $i=1,\ldots,m$, and $m$ is the number of LQP-subtrees. Additionally, $\phi_j$ is the LQP-sub predictive model of the $j$-th objective, where $j=1,\ldots,k$. The function $\Lambda$ is a general mapping from LQP-subtree-level values to query-level objective values, following the calculation of the topological structure of LQP.
}





==> checkpoint-231115/Qi_initial_optimizer/definitions_and_Intuitions.tex <==
\section{Definitions and intuitions}

%The following is based on the current proposal entitled \textbf{2-step divided-and-conquer MOO method}. 

\subsection{Formal Definitions} 

We introduce our associated terminology here.

{\definition{\textbf{Tuning Parameter}}: A tuning parameter is a configuration variable that decides the performance of a big data system for an application.} 

A Spark physical plan of a query could be represented as a Directed Acyclic Graph (DAG) of stages. Any arbitrary stage $s$ has two types of tuning parameters, i.e. \textbf{Shared Parameters} $\bm{\theta_q}$ and \textbf{Stage-specific Parameters} $\bm{\theta_s}$, where $\bm{\theta_q} \in \mathbb{R}^{d_1}$ should be the same among all stages, and $\bm{\theta_s} \in \mathbb{R}^{d_2}$ could be different for different stages. So, the parameter space of a stage includes $d_1 + d_2$ parameters, and the parameter space of a query includes $d_1 + |S| * d_2$ parameters when there are $|S|$ stages. 

{\definition{\textbf{Configuration}}: A configuration is a constant vector, which sets a specific value for each tuning parameter under a set of fixed and ordered parameters. The \textbf{Configuration Space} is the set including all possible configurations.} %refer to the definition from the UDO paper

For example, a configuration for the query with $|S|$ stages is a ($d_1 + |S| * d_2$)-dim constant vector and a configuration for an arbitrary stage is a ($d_1 + d_2$)-dim constant vector. 

Our goal is to find the Pareto optimal configurations for a query by considering multiple user-specified objectives. This query-level MOO problem could be addressed in either \textbf{Query-level tuning} or \textbf{Stage-level tuning}.

{\definition{\textbf{Query-level tuning}}: Query-level tuning solves the query-level MOO problem directly, which treats ($\bm{\theta_q}, \bm{\theta_1}, ..., \bm{\theta_{|S|}}$) for all $|S|$ stages in a query as the input, and its output is the Pareto optimal configurations for this query. When $|S|$ is large, its parameter space could be large (e.g. hundreds or thousands of parameters).}

By query-level tuning, we can define a general query-level MOO problem as follows:

{\definition{\textbf{General Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:1_general_query_mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})=& {\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Psi_1(\bm{\alpha}, \bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}}) \\ 
			...\\
			F_k(\bm{\theta}) = \Psi_k(\bm{\alpha}, \bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}})
			\end{array}
			\right]} \\
		\nonumber s.t. & 
		& \bm{\theta_q} \in  \mathbb{R}^{d_1} \quad \bm{\theta_s} \in  \mathbb{R}^{d_2}, \quad s = 1,..., |S|\\
		\end{eqnarray}
}}

\noindent{ 
where we denote $\bm{\alpha}$ as the non-decision variables required in the query-level predictive model, and $\bm{\theta} = [\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}}]$ is configurations for the whole query, $\Psi_j$ is the query-level predictive model for $j$-th objective, where $j=1,...,k$.}

{\definition{\textbf{Stage-level tuning}}: Stage-level tuning addresses the MOO problem within a stage, and its output is the Pareto optimal configurations for each stage, where its parameters space is fixed with $d_1 + d_2$ parameters. To achieve the query-level Pareto optimal configurations, it is necessary to design an algorithm to optimally compose stage-level configurations into the query level.}

By stage-level tuning, we can define the above query-level MOO in \ref{eq:1_general_query_mult_obj_opt_def} as the following:

{\definition{\textbf{Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:sep_query_mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})={\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Lambda_1(\Phi_1(\bm{\alpha_1}, \bm{\theta_q}, \bm{\theta_1}),...,\Phi_1(\bm{\alpha_{|S|}}, \bm{\theta_q},\bm{\theta_{|S|}})) \\ 
			...\\
			F_k(\bm{\theta}) = \Lambda_k(\Phi_k(\bm{\alpha_1}, \bm{\theta_q},\bm{\theta_1}),...,\Phi_k(\bm{\alpha_{|S|}},\bm{\theta_q},\bm{\theta_{|S|}}))
			\end{array}
			\right]} \\
		\nonumber s.t. & \bm{\theta_q} \in  \mathbb{R}^{d_1} \quad\bm{\theta_s} \in  \mathbb{R}^{d_2}, s = 1, ..., |S|\\
		\end{eqnarray}
}}

\noindent{
where we denote $\bm{\alpha_s}$ as the non-decision variables required in the predictive model of the stage $s$, $\bm{\theta} = [\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}}]$ is configurations for all stages within a query, $\Phi_j$ is the stage-level predictive model of  $j$-th objective, where $j=1,..,k$. $\Lambda_j$ is the general function mapping from the stage-level values to the $j$-th query-level objective values, which follows the calculation of the topological order of DAG.}

For an arbitrary stage $s$, after stage-level tuning, its Pareto optimal configurations for ($\bm{\theta_q}, \bm{\theta_s}$) have the following properties.

\minip{Property 1:} For optimal $\bm{\theta_q}$, under different stages, optimal $\bm{\theta_q}$ after \textbf{stage-level tuning} could be different as the non-decision variables $\bm{\alpha_s}$ of different stages are different.

\minip{Property 2:} For optimal $\bm{\theta_s}$ under a fixed $\bm{\theta_q}$ configuration,

\begin{itemize}
	\item Optimal $\bm{\theta_s}$ could have multiple configurations as tuning $\bm{\theta_s}$ under a fixed $\bm{\theta_q}$ configuration is a MOO problem.
	\item For the same stage, due to different $\bm{\theta_q}$ configurations, optimal $\bm{\theta_s}$ configurations could be different.
	\item Under different stages with a fixed $\bm{\theta_q}$, optimal $\bm{\theta_s}$ configurations could be different as the non-decision variables $\bm{\alpha_s}$ of different stages are different.
\end{itemize}

The above properties and the requirement that $\bm{\theta_q}$ configurations should be the same among all the stages make
\textbf{stage-level tuning} more complex with different control on $\bm{\theta_q}$ and $\bm{\theta_s}$.
While this could be addressed by an efficient algorithm design, named \textbf{2-step divided and conquer MOO approach}, which will be explained in later sections. The following section will illustrate the intuitions related to the \textbf{stage-level tuning} with theoretical analysis.

\subsection{Intuitions}

\minip{Intuition 1:} \textbf{Stage-level tuning} could provide a warm-start to achieve the query-level Pareto optimal.
%\begin{figure}
%     \centering
%     \begin{subfigure}[b]{}
%%         \centering
%     \includegraphics[height=3.5cm,width=3.3cm]{figs/intuitions_query_moo/local_pareto_stage_1.png}
%         \caption{Stage 1}
%         \label{fig:local_pareto_stage_1}
%     \end{subfigure}
%%     \vfill
%     \begin{subfigure}[b]{}
%%         \centering
%         \includegraphics[height=3.5cm,width=3.3cm]{figs/intuitions_query_moo/local_pareto_stage_2.png}
%         \caption{Stage 2}
%         \label{fig:local_pareto_stage_2}
%     \end{subfigure}
%     \caption{Stage-level Pareto solutions after Stage-level tuning}
%      \label{fig:eg_stage_tuning}
%\end{figure}


\begin{figure}
  \centering
  \begin{tabular}{ll}
		\subfigure[\small{Stage 1}]
		{\label{fig:local_pareto_stage_1}\includegraphics[width=.45\linewidth]{figs/intuitions_query_moo/local_pareto_stage_1.png}}
%		\vspace{-0.02in}
%		\\
		\subfigure[\small{Stage 2}]
		{\label{fig:local_pareto_stage_2}\includegraphics[width=.45\linewidth]{figs/intuitions_query_moo/local_pareto_stage_2.png}} 					  
  \end{tabular}
  \vspace{-0.2in}
  \captionof{figure}{\small{Example of stage-level Pareto solutions after Stage-level tuning}}
  \label{fig:eg_stage_tuning}
\end{figure}

\minip{Example} ~

Figure \ref{fig:eg_stage_tuning} shows an example of a query with 2 stages. Each subplot shows the objective space of a stage, which is bounded by Utopia and Nadir points, where Utopia achieves the minimum values in both latency and cost objectives, and Nadir achieves the maximum. Each blue point is a Pareto optimal point returned after stage-level tuning. 

We denote the $\bm{\theta_q}$ configurations from the Pareto optimal solutions of stage $s$ as the $\bm{cq_s}$, where $s=1,2$ in Figure \ref{fig:eg_stage_tuning}. For example, in stage 1, $\bm{cq_1}=\{\bm{\theta_{q1}}, \bm{\theta_{q2}}\}$; in stage 2, $\bm{cq_2}=\{\bm{\theta_{q1}}, \bm{\theta_{q2}}, \bm{\theta_{q3}}\}$. 
As the $\bm{\theta_q}$ configurations should be the same among all stages, we denote the union of $\bm{cq_s}$ as a $\bm{\theta_q}$ candidate set $\bm{\Theta^{cand}_q}=\{ \bm{\theta^*_{qi}}, i=1,...,|\bm{\Theta^{cand}_q}| \}$, which provides a global set for all stages. In Figure \ref{fig:eg_stage_tuning}, $\bm{\Theta^{cand}_q}=\{ \bm{\theta_{q1}}, \bm{\theta_{q2}}, \bm{\theta_{q3}} \}$, where $\bm{\theta^*_{q1}}=\bm{\theta_{q1}}, \bm{\theta^*_{q2}}=\bm{\theta_{q2}}, \bm{\theta^*_{q3}}=\bm{\theta_{q3}}$. 
We denote the $j$-th optimal stage-specific configuraion under $\bm{\theta^*_{qi}}$ for stage $s$ as $\bm{\theta^*_{sij}}$, where $j=1,...,p_i$, and $p_i$ is the number of optimal stage-level specific configurations under $\bm{\theta^*_{qi}}$. For example, in stage 1, under $\bm{\theta_{q1}}$, $p_1=2$, the second optimal $\bm{\theta_s}$ configuration is $\bm{\theta^*_{112}}$. 


\begin{figure}
  \centering
  \begin{tabular}{ll}
		\subfigure[\small{Stage 1}]
		{\label{fig:global_pareto_stage_1}\includegraphics[width=.45\linewidth]{figs/intuitions_query_moo/global_pareto_stage_1.png}}
%		\vspace{-0.02in}
%		\\
		\subfigure[\small{Stage 2}]
		{\label{fig:global_pareto_stage_2}\includegraphics[width=.45\linewidth]{figs/intuitions_query_moo/global_pareto_stage_2.png}} 					  
  \end{tabular}
  \vspace{-0.2in}
  \captionof{figure}{\small{Example of stage-level Pareto solutions under $\bm{\Theta^{cand}_q}$}}
  \label{fig:eg_stage_space_division}
\end{figure}

Since all the stages should share the same $\bm{\theta_q}$ configurations, the above example is updated in Figure \ref{fig:eg_stage_space_division} under $\bm{\Theta^{cand}_q}$. Based on the $\bm{\Theta^{cand}_q}$ and their corresponding optimal $\bm{\theta_s}$ configurations, the objective space could be divided into different regions (e.g. the red region in Figure \ref{fig:global_pareto_stage_1}) by considering query-level optimality. 

The query-level optimality is decided by an \textbf{Optimality-boundary point} in each stage. The intuition of \textbf{Optimality-boundary point} is to identify and prune sub-regions which is impossible to contribute to the query-level Pareto optimal configurations. For example, the green point $P_1$ in Figure \ref{fig:global_pareto_stage_1} is the \textbf{Optimality-boundary point} of stage 1. The optimality proof related to the divided regions is presented in the later sub-section.

\textbf{Optimality-boundary point} of a stage is determined by \textbf{Optimality-boundary latency of stage $s$} (i.e. $lat_{ob}^s$) and \textbf{Optimality-boundary cost of stage $s$} (i.e. $cost_{ob}^s$),
where $lat_{ob}^s=\max(f_{lat}(\min(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}|j=1,...,p_i)|i=1,...,|\bm{\Theta^{cand}_q}|)$, $cost_{ob}^s=\max(f_{cost}(\min(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}|j=1,...,p_i)|i=1,...,|\bm{\Theta^{cand}_q}|)$ with stage-level latency and cost predictive models $f_{lat}$ and $f_{cost}$ respectively.

For example, in stage 1, under a specific $\bm{\theta^*_{qi}}$ configuration, we denote the latency and cost of one of the points as 

\begin{equation}
	\begin{split}
	lat_{sij} & = f_{lat}(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}), j=1,...,p_i\\
	cost_{sij}& = f_{cost}(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}), j=1,...,p_i
	\end{split}
\end{equation}
	
%$lat_{sij}=f_{lat}(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}|j=1,...,p_i)$
%
%$cost_{sij}=f_{cost}(\bm{\theta^*_{qi}}, \bm{\theta^*_{sij}}|j=1,...,p_i)$. 

Then the $lat_{ob}^1$ and $cost_{ob}^1$ are as the following:

\begin{equation}
	\begin{split}
	lat_{ob}^1 & = \max(\min(lat_{111}),\min(lat_{121}),\min(lat_{131}))\\
	& = lat_{111}
	\end{split}
\end{equation}

\begin{equation}
	\begin{split}
	cost_{ob}^1 & = \max(\min(cost_{111}),\min(cost_{121}),\min(cost_{131}))\\
	& = cost_{131}
	\end{split}
\end{equation}
%$lat_{ob}^1=max(min(lat_{111}),min(lat_{121}),min(lat_{131}))$
%
%$cost_{ob}^1=max(min(cost_{111}), min(cost_{121}),min(cost_{131}))$. 

Where the point $P_1$ is determined as the \textbf{Optimality-boundary point} since it achieves both $lat_{ob}^1$ and $cost_{ob}^1$.

Similarly in stage 2, the $lat_{ob}^2$ and $cost_{ob}^2$ are as the following:

\begin{equation}
	\begin{split}
	lat_{ob}^2 & = \max(\min(lat_{211},lat_{212}),\min(lat_{221},lat_{222}), \min(lat_{231}))\\
	& = \max(lat_{211}, lat_{222}, lat_{231})\\
	& = lat_{222}
	\end{split}
\end{equation}

\begin{equation}
	\begin{split}
	cost_{ob}^2 & = \max(\min(cost_{211},cost_{212}),\min(cost_{221},cost_{222}), \min(cost_{231}))\\
	& = \max(cost_{211}, cost_{221}, cost_{231})\\
	& = cost_{231}
	\end{split}
\end{equation}

%$lat_{ob}^2=max(min(lat_{111},lat_{112}),min(lat_{121},lat_{122}), min(lat_{111}))$
%
%$cost_{ob}^2=max(min(cost_{111},cost_{112}),min(cost_{121},cost_{122}), min(cost_{111}))$. 

Where the point $P_2$ is determined as the \textbf{Optimality-boundary point} since it achieves both $lat_{ob}^2$ and $cost_{ob}^2$.

Based on the \textbf{Optimality-boundary point}, the objective space of each stage could be split into different sub-regions, where solutions located in the red regions (e.g. $\Omega_1$ and $\Omega_2$ in Figure \ref{fig:eg_stage_space_division}) can be proved to be dominated in the query-level.


\todo{TODO: intuitions related to "missing point", the current proposal needs to be improved further}


\subsubsection{Theoretical Analysis} ~

\begin{proposition}
	For any arbitrary stage $s$, the optimality-boundary point $P_s$ is dominated by stage-level optimal solutions constructed by all $\bm{\theta_q} \in \bm{\Theta^{cand}_q}$.
\end{proposition}

\begin{proof}
In any stage $s$ of an arbitrary DAG, the optimality-boundary point $P_s$ is dominated by stage-level optimal solutions $f^s$ constructed by any $\bm{\theta_q} \in \bm{\Theta^{cand}_q}$. 

Suppose $P_s$ is dominant or non-dominated with $f^s$. There must be $P_s$ has lower latency and cost than $f^s$, which is impossible as $P_s$ achieves maximum latency and cost among stage-level optimal solutions constructed by all $\bm{\theta_q} \in \bm{\Theta^{cand}_q}$.
Then the proof is concluded.  

\end{proof}

\begin{proposition}
	For all stages, solutions located in the red region cannot contribute to query-level Pareto optimal solutions.
\end{proposition}

\begin{proof}
In any stage $s$ of an arbitrary DAG, the dominated solution $f^s$ (red area) is dominated by ${f'}^s$ with any arbitrary $\bm{\theta_q}$; query-level solution $F$ built from $f^s$, $F$ built from ${f'}^s$. 

Suppose $F$ is non-dominated with $F'$ or dominates $F'$. There must be at least one $f^s$ with lower latency or cost than ${f'}^s$, which is impossible and concludes the proof.  

\end{proof}


\cut{
\begin{proposition}
	For all stages, solutions located in each of the yellow (or brown) regions cannot dominate the query-level non-dominated solutions constructed from the stage-level optimal $\bm{\theta}_q$.
\end{proposition}

\begin{proof}
in any stage $s$ of an arbitrary DAG, the dominated solution $f^s$ (an arbitrary yellow region) is dominated by ${f'}^s$; query-level solution $F$ built from $f^s$, $F$ built from ${f'}^s$. 

Suppose $F$ dominates $F'$. There must be at least one $f^s$ with lower latency and cost than ${f'}^s$, which is impossible and concludes the proof.  

\end{proof}

}


==> checkpoint-231115/Qi_initial_optimizer/query_moo_algo.tex <==
\section{Improved MOO Algorithm for the Query-level}

In this algorithm design, we optimize latency and cost together in the query-level MOO problem. 

\todo{
Assume there are $S$ stages, and $m$ parameters to be tuned for each stage. Generally, the optimal configuration for the query-level MOO problem includes $S * m$ parameters.
} 

The stage-level predictive model takes the embedding of the subquery plan, the input meta, and the cluster system state. We assume that the cluster system state is invariant during the algorithm processing. Thus, given the query, the Pareto solutions (with corresponding configurations) of all stages can be obtained in advance. Currently, we call it as the static query-level MOO.

The Algorithm \ref{alg:improved_query_level_moo} is the corresponding pseudo-code for the static query-level MOO with objectives such as latency and cost.

\begin{algorithm}[t]
	\caption{Query-level MOO}
	\label{alg:improved_query_level_moo}
	\small
	\begin{algorithmic}[1]  
		\REQUIRE {$Q, \bm{\Theta^q}, \Phi_i, t$, $\forall i\in [1,k]$}.
%		\STATE $w_l = 0, w_c = 1, \bm{\Theta}=[], \bm{f}=[]$ %Initialize weights for latency and cost
        \STATE $\bm{\Theta}=[], \bm{f}=[]$
        \STATE \% {\textit{Get Pareto solutions for all stages}}
		\FOR {$s$ \textbf{in} $\bm{S}$}
                \STATE ${\bm{f}^s}$, ${\bm{\Theta}^s}$ = stage\_moo(t, $\Phi$,$\bm{\Theta^q}$, $\bm{\Theta^s}$)
%                \STATE ${\bm{f}^s}^*$, ${\bm{\Theta^s}}^*$ = choose\_optimal(${\bm{f}^s}$, ${\bm{\Theta^s}}$, $w_l$, $w_c$)
%                \STATE t = update\_timestamp(t, $s$, $Q$, ${\bm{f}^s}^*$)
                \STATE $\bm{\Theta}$.append(${\bm{\Theta^s}}$), $\bm{f}$.append(${\bm{f}^s}$)
            \ENDFOR
            \STATE \% \textit{Simplify the DAG graph}
            \STATE $\bm{V}$, $\bm{f}'$, $\bm{\Theta}'$ = transform\_DAG($Q$, $\bm{f}$, $\bm{\Theta}$)
            \STATE \% \textit{Simplify the DAG graph}
            \STATE $\bm{F}$, $\bm{\Theta}$ = optimize($\bm{V}$, $\bm{f}'$, $\bm{\Theta}'$)
            \RETURN $\bm{F}$, $\bm{\Theta}$
	\end{algorithmic}
\end{algorithm}

\begin{figure*}
\centering
\captionsetup{justification=centering}
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[height=5cm,width=4.5cm]{figs/dag_transformation_eg.png}
  \captionof{figure}{\small{An example of a DAG transformation}}
  \label{fig:dag_transformation_example}
\end{minipage}
\begin{minipage}{.48\textwidth}
  \centering
  \includegraphics[height=5cm]{figs/query_example.png}
  \captionof{figure}{\small{An example of a Spark query graph}}
  \label{fig:query_example}
\end{minipage}
\end{figure*}

Lines 1-8 are the same as that in the previous algorithm design, which generates the Pareto solutions for all stages. The start time of the child stages is determined by the finish time of their parent stages, while each stage could have multiple Pareto solutions with different latency values. To minimize the cost, the start time of the child stages are determined as the maximum finish time among the Pareto solutions of its parent stages. The finish time of a stage is the sum of its start time and its latency.

Based on the Pareto solutions of all stages in the query graph, line 10 transforms the DAG graph into the one with serial stages, like shown in Figure \ref{fig:dag_transformation_example}, and the details are described in the Algorithm \ref{alg:transform_dag}. And line 11 optimizes latency and cost by using existing MOO algorithms (e.g. weighted sum (WS))based on the transformed DAG.

\minip{Example}

Assume the Pareto solutions (e.g. [latency, cost])for each stage in the Figure \ref{fig:dag_transformation_example} are obtained as the following after lines 1-8: 

\noindent{Stage 1: $[5,20],[8,17],[10,15]$ \\
Stage 2: $[4,30],[6,10]$ \\
Stage 3: $[8,8],[9,7]$ \\
Stage 4: $[7,9],[15,5]$ \\
Stage 5: $[1,10],[10,1]$ \\
Stage 6: $[17,15],[20,10]$ \\
Stage 7: $[30,20],[40,10]$ \\}

After DAG transformation, stage $1'$ should includes the same output as all stages of 1, 2, 3 and 4. For latency, that is the maximum between the finish time of stage 3 and 4, and cost is the sum of all 4 stages. In the example, there are 6 finish time values of stage 3, obtained by the combination of 3 solutions in stage 1 and stage 3, i.e. $5+8=13, 5+9=14, 8+8=16, 8+9=17, 10+8=18, 10+9=19$. Similarly, there are 4 finish time values of stage 4, i.e. $11, 13, 19, 21$. So, stage $1'$ will include $13, 14, 16, 17, 18, 19, 21$ as the latency values. Accordingly, their cost values are $47, 46, 44, 43, 42, 41, 37$, where the combination is the Pareto solutions of stage $1'$, i.e. $[13,47],[14,46],[16,44],[17,43],[18,42], [19,41],[21,37]$, and it has enumerated all the latency values before stage 5.

After getting the serial stages, both the query-level latency and cost take the sum over all stages. WS will guarantee to return Pareto optimal solutions, where the proof is the same as the optimality proof in the General Hierarchical MOO.

\begin{algorithm}[t]
    \caption{DAG\_transformation}
    \label{alg:updated_dag_transformation}
    \small
    \begin{algorithmic}[1]  
        \REQUIRE {$\bm{Q}$, each stage $\bm{s}$ has its Pareto set $\bm{s}.po$ (i.e. $\bm{f^s}$), configurations $\bm{s}.conf$ (i.e. $\bm{\Theta} = [\bm{\Theta^q, \Theta^s}]$), parent and child nodes $\bm{s}.parent$, $\bm{s}.child$, $s=1,..,S$}.
        \STATE get stage queue $\bm{S}$ following the topological order
        \STATE branch\_dict = \{\}, serial\_nodes\_dict = \{\}, merged\_nodes = [ ], final\_nodes\_list = [ ]
        \WHILE{$\bm{S}$ is not empty}
            \STATE $\bm{s} = \bm{S}.pop$
            \IF{$\bm{s}$ is not exit}
                \IF {$s$ in merged\_nodes}
                    \STATE keys = $\bm{s}.parent$, 
                    \STATE $\bm{v}.po, \bm{v}.conf$ = merge\_branches(branch\_dict[keys])
                    \STATE $\bm{v}.child$ = $\bm{s}$, $\bm{v}.parent$ = [ ]
                    \STATE serial\_nodes\_dict.remove([keys]), serial\_nodes\_dict[$\bm{s}.id$] = [$\bm{v}$, $\bm{s}$]
                    \IF{$len(\bm{s}.child.parent) > 1$}
                        \STATE ind = $\bm{s}$.parent
                        \STATE branch\_dict[$\bm{s}$.id] = serial\_nodes\_dict[ind]
                    \ENDIF
                \ELSE 
                    \IF{any child with $len(\bm{s}.child.parent) > 1$}
                        \IF{$\bm{s}.child$ is not in merged\_nodes}
                            \STATE merged\_nodes.$append(\bm{s}.child)$
                        \ENDIF
                        \IF{$s$ is entry}
                            % \STATE branch\_dict[$\bm{s}.id$] = [$\bm{s}$]
                            \STATE serial\_nodes\_dict[$\bm{s}.id$]$.append(\bm{s})$
                        \ELSE
                            % \STATE ind = find\_key($\bm{s}$, serial\_nodes\_dict)
                            % \STATE branch\_dict[$\bm{s}$.id] = serial\_nodes\_dict[ind]$.append(\bm{s})$
                            \STATE ind = $\bm{s}$.parent
                            \STATE serial\_nodes\_dict[ind]$.append(\bm{s})$
                        \ENDIF
                        \STATE branch\_dict[$\bm{s}$.id] = serial\_nodes\_dict[ind]
                    \ELSE 
                        \STATE update\_serial\_nodes($\bm{s}$, serial\_nodes\_dict)
                    \ENDIF
                \ENDIF
            \ELSE %{$s$ is the exit stage}
                \STATE update\_serial\_nodes($\bm{s}$, serial\_nodes\_dict)
                \STATE final\_nodes\_list$.append(\bm{s})$
            \ENDIF
        \ENDWHILE 
        \RETURN final\_nodes\_list
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{update\_serial\_nodes}
    \label{alg:updated_serial_nodes}
    \small
    \begin{algorithmic}[1]  
        \REQUIRE {$\bm{s}$, serial\_nodes\_dict}.
        \STATE ind = $\bm{s}$.parent
        \STATE updated\_list = serial\_nodes\_dict[ind]$.append(\bm{s})$
        \STATE serial\_nodes\_dict.remove([ind]) 
        \STATE serial\_nodes\_dict.add($\bm{s}.id$:updated\_list)
        \RETURN final\_nodes\_list
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{merge\_branches}
    \label{alg:merge_branches}
    \small
    \begin{algorithmic}[1]  
        \REQUIRE {branch\_dict, ws\_pairs}.
        \STATE branch\_list = [ ]
        \FOR{id \textbf{in} branch\_dict.keys}
            \STATE create a new node $\bm{v}$
            \STATE $\bm{v}.po$, $\bm{v}.conf$ = optimize(branch\_dict[id], ws\_pairs)
            \STATE branch\_list$.append(\bm{v})$
        \ENDFOR
        \STATE po, conf = raa\_path(branch\_list)
        \RETURN po, conf
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{optimize}
    \label{alg:optimize}
    \small
    \begin{algorithmic}[1]  
        \REQUIRE {nodes\_list, ws\_pairs}.
        \STATE PO = [ ], conf = \{\}
        \FOR{$[w_l, w_c]$ \textbf{in} ws\_pairs}
            \STATE po\_n = [ ], conf\_n = \{\}
            \FOR{$\bm{n}$ \textbf{in} nodes\_list}
                \STATE ${\bm{n}.po}'$ = normalize($\bm{n}.po$)
                \STATE opt\_ind, opt\_ws = minimize\_ws($[w_l, w_c]$, ${\bm{n}.po}'$)
                \STATE results$.append$($\bm{n}.po$[opt\_ind])
                \STATE conf\_n[$\bm{n}.id$] = $\bm{n}.conf$
            \ENDFOR
            \STATE PO$.append$(sum(results)), conf$.append$(conf\_n)
        \ENDFOR
        \RETURN PO, conf
    \end{algorithmic}
\end{algorithm}

\subsection{DAG transformation}
After getting Pareto solutions for all stages, we can further simplify the DAG graph. For example, in Figure \ref{fig:dag_transformation_example}, stages 1 and 3 are in the same branch, while stages 2 and 4 are in the other one. After the Pareto solutions of stages 1 and 3 are obtained, we can enumerate all the results of stage 3, so as stage 4. Then stage 5 takes the results of stages 3 and 4 together to continue the calculation for the following DAG graph. So, if there is one node with all the results of stages 3 and 4, it is reasonable to replace stages 1, 2, 3, and 4 with this node, because the results passed to stage 5 are the same.

Thus, the intuition of this DAG transformation is to merge branches of the graph to simplify it as a serial graph. The pseudo-code is shown in Algorithm \ref{alg:updated_dag_transformation}.

\minip{Algorithm description}
Algorithm \ref{alg:updated_dag_transformation} takes the query as input, where each stage has its Pareto solutions, configurations, parent and child nodes. Lines 1-2 initialize a stage queue $\bm{S}$ which follows a topological order. The \textit{branch\_dict} is a dictionary whose keys are stage ids, and values are lists of branches, where each element is a stage. \textit{serial\_nodes\_dict} indicates the current serial stages (or nodes), and it will be updated after the branches are merged. Each key is a stage id, whose value is a list of serial nodes. The aim is to keep the latest serial nodes of the transforming graph.  \textit{merged\_nodes} indicates a list of nodes who have multiple parent nodes (e.g. stages 5, 6, 10, 11 in Figure \ref{fig:query_example}).  \textit{final\_nodes\_list} is a list that includes one (i.e. one exit stage) or more serial nodes lists (i.e. multiple exit stages).

The DAG transformation is addressed within the \textit{while} loop, which checks whether all the stages are processed or not. If not, line 4 pops out one stage by following the query topological order. If it is not an exit stage, there is at least one child stage, so there are two cases to indicate whether the current stage is on a branch to be merged further (line 6), or it is on a serial branch (line 15). 

Line 6 checks whether the current stage is a merged node . If so, it means all its parents are finished and will be merged to create a new node. Line 7 finds out the keys of branches to be merged, and line 8 merges these branches further to return a new node with the updated Pareto solution, configurations, parent and child nodes. The details of how to merge are shown in Algorithm \ref{alg:merge_branches}. After merging, any serial nodes of the merged branches are removed from the \textit{serial\_nodes\_dict}, and the new node along with the current stage are added in the \textit{serial\_nodes\_dict} with the key of the current stage id (line 10). The \textit{branch\_dict} is updated with the new node (line 11-14).

Otherwise, it will update the \textit{branch\_dict}, \textit{merged\_nodes} and \textit{serial\_nodes\_dict} further. Line 16 further checks whether the child of the current stage has multiple parent (e.g. node 5 in Figure \ref{fig:query_example}). If so, it means there are multiple branches to be merged at the child stage. Lines 17-19 updates the \textit{merged\_nodes} without duplication. lines 20-25 update the \textit{branch\_dict}. If not, it means it is a serial branch. And line 27 updates the \textit{serial\_nodes\_dict} by keeping the key as the end stage of the branch, and details are shown in Algorithm \ref{alg:updated_serial_nodes}.

If it is an exit stage, there is no child stage, so it is used to update the current \textit{serial\_nodes\_dict} and put it into the \textit{final\_nodes\_list} (lines 30-34).  

Finally, line 32 returns the \textit{final\_nodes\_list} as the transformed DAG, which may include one or multiple serial node lists.

\minip{Example of Algorithm \ref{alg:updated_dag_transformation}}
Let's take a more complex query in Figure \ref{fig:query_example} as an example. Assume the stages with topological order as $[2, 3, 1, 5, 4, 7, 6, 8, 9, 10, 11, 12]$.

Now $\bm{S}$ is not empty, then stage 2 is obtained from the queue. It is an entry stage. Currently, the \textit{merged\_nodes} list is empty, so it jumps to line 11. its child is stage 5, which has 2 parent nodes (i.e. stages 1 and 2). As the \textit{merged\_nodes} list is empty, stage 5 is added and the \textit{merged\_nodes} is updated as $[5]$. Since stage 2 is an entry stage, it executes line 16, and updates the current \textit{serial\_nodes\_dict} and \textit{branch\_dict} as $\{"2":[2]\}$. Then it continues to the next stage, i.e. stage 3.

Stages 3 and 1 are executed similarly to stage 2. And we have the updated \textit{serial\_nodes\_dict} and \textit{branch\_dict} as $\{"2":[2], "3":[3], "1":[1]\}$. And the \textit{merged\_nodes} is updated as $[5, 6]$.

Stage 5 is not the exit, and it is in the \textit{merged\_nodes} list. Then, line 7 finds the parents of stage 5, which are stages 1 and 2 respectively. Line 8 merges the branches of $[1]$ and $[2]$, and creates a new node $v\_1$ with the updated Pareto solutions, configurations, parent and child nodes. Then the \textit{serial\_nodes\_dict} is updated as $\{"3":[3], "5":[v\_1, 5]\}$.

After that, it is stage 4, similarly, as stage 2, it updates the \textit{serial\_nodes\_dict} as $\{"3":[3], "5":[v\_1, 5], "4":[4]\}$, and the \textit{branch\_dict} as $\{"2":[2], "3":[3], "1":[1], "4":[4]\}$.

Then, stage 7 comes. It is not the exit and not in the merged\_nodes list. Stage 7 has a child, i.e. stage 10, which has 2 parent nodes (i.e. stages 7 and 8). Then line 13 updates \textit{merged\_nodes} list with stage 10 as $[5, 6, 10]$. Stage 7 is not an entry stage, since its parent node is stage 5, then the serial path that stage 7 belongs to is $[v\_1, 5]$. So it updates the \textit{serial\_nodes\_dict} as $\{"3":[3], "5":[v\_1, 5], "4":[4], "7":[v\_1, 5, 7]\}$, and the \textit{branch\_dict} as $\{"2":[2], "3":[3], "1":[1], "4":[4], "7":[v\_1, 5, 7]\}$.

The next is stage 6. It is not the exit but in the merged\_nodes list. Similarly to stage 5, it merges the branches of $[3]$ and $[4]$, and creates a new node $v\_2$ with the updated Pareto solutions, configurations, parent and child nodes. Then the \textit{serial\_nodes\_dict} is updated as $\{"6":[v\_2, 6]\}$.

Next is stage 8. Similarly to stage 7, it has a child, i.e. stage 10, which has already been included in the \textit{merged\_nodes} list. Stage 8 is not an entry stage, since its parent node is stage 5, then the serial path that stage 8 belongs to is $[v\_1, 5]$. So the \textit{branch\_dict} is updated as $\{"2":[2], "3":[3], "1":[1], "4":[4], "7":[v\_1, 5, 7], "8":[v\_1, 5, 8]\}$.

Then, it is stage 9. It is not the exit and not in the \textit{merged\_nodes} list. Its child is stage 11, which has 2 parents (i.e. stages 10 and 9). Then line 13 updates \textit{merged\_nodes} list with stage 11 as $[5, 6, 10, 11]$. Stage 9 is not an entry stage, since its parent node is stage 6, then the serial path that stage 9 belongs to is $[v\_2, 6]$. So the the \textit{branch\_dict} as $\{"2":[2], "3":[3], "1":[1], "4":[4], "7":[v\_1, 5, 7], "8":[v\_1, 5, 8], "9":[v\_2, 6, 9]\}$.

Then, it is stage 10. It is not the exit but in the \textit{merged\_nodes} list. The parents of stage 10 are stages 7 and 8. So it merges the branches of $[v\_1, 5, 7]$ and $[v\_1, 5, 8]$, and creates a new node $v\_3$ with the updated Pareto solutions, configurations, parent and child nodes. Then the \textit{serial\_nodes\_dict} is updated as $\{"10":[v\_3, 10]\}$. Stage 11 is the child of stage 10, which has 2 parent nodes. So the \textit{branch\_dict} is updated as $\{"2":[2], "3":[3], "1":[1], "4":[4], "7":[v\_1, 5, 7], "8":[v\_1, 5, 8, "9":[v\_2, 6, 9], "10":[v\_3, 10]\}$.

Then it is stage 11. It is not the exit but in the \textit{merged\_nodes} list. The parents of stage 11 are stages 10 and 9. So it merges the branches of $[v\_3, 10]$ and $[v\_2, 6, 9]$, and creates a new node $v\_4$ with the updated Pareto solutions, configurations, parent and child nodes. Then the \textit{serial\_nodes\_dict} is updated as $\{"11":[v\_4, 11]\}$.

Finally, it comes to stage 12. It is the exit stage. And the \textit{serial\_nodes\_dict} is updated as $\{"12":[v\_4, 11, 12]\}$ and added to the \textit{final\_nodes\_list} which is returned as the transformed DAG.

\todo{how complex the graph will be? e.g. the case of stage 5, 7, 8; or imagine stage 6 is also the child of stage 1)}

\subsubsection{Complexity analysis}

Assuming the complexity of line 3 is $\lambda$, the maximum number of Pareto solutions for each stage (or node) is $P_{max}$. The complexity of getting the initial Pareto solutions for all stages (lines 1-8) is $O(S * (\lambda + P_{max})$.

Assume the maximum number of Pareto solutions for each node during the DAG transformation is $P_{max}^v$. For the DAG transformation, assume there are $\alpha$ merged nodes, and for each merged node, there are $\beta$ branches. In each branch, there are at most $d$ nodes. DAG transformation includes Algorithm \ref{alg:merge_branches}, where Algorithm \ref{alg:merge_branches} includes Algorithm \ref{alg:optimize} and \textit{raa\_path}. The complexity of Algorithm \ref{alg:optimize} is $O(W * d * P_{max}^v)$. Then, the complexity of lines 2-6 in Algorithm \ref{alg:merge_branches} is $O(\beta * W * d * P_{max}^v)$. Suppose in each branch, the maximum number of solutions is $P_{max}^b$. The complexity of \textit{raa\_path} is $O(\beta * P_{max}^b * log (\beta * P_{max}^b)$.
So, the complexity of Algorithm \ref{alg:merge_branches} is $O(\beta * W * d * P_{max}^v) + O(\beta * P_{max}^b * log (\beta * P_{max}^b)$.

Thus, for the query, the complexity of the DAG transformation is $O(\alpha * (O(\beta * W * d * P_{max}^v) + O(\beta * P_{max}^b * log (\beta * P_{max}^b))$.

After transformation, assume the number of serial nodes is $d$. If it applies WS, its complexity is $O(W * d * P_{max}^v)$, where we denote the number of weight settings is $W$.

\subsubsection{Optimality analysis}
Lines 1-8 generate the Pareto optimal solutions for all stages. For each stage, the optimality is determined by the stage-level MOO approach used.

DAG transformation (i.e. line 10) guarantees that the transformed node returns a subset of Pareto solutions for all branches to be merged. 

If line 12 applies WS, it guarantees to return a subset of query-level Pareto solutions.

Overall, the improved algorithm guarantees to return a subset of query-level Pareto solutions.

\minip{Optimality Proof}

The Algorithm \ref{alg:improved_query_level_moo} mainly includes 3 operations: 1) the stage-level MOO method (line 4); 2) DAG transformation (line 10); 3) optimization over a serial node list (line 12).

The following are the optimality analysis for operations 2) and 3) based on the stage-level Pareto solutions obtained by 1).

Since the DAG transformation includes operation 3). Now we first prove for this case: when there are $d$ serial nodes, where each node has a Pareto set and its corresponding configurations. 

\begin{lemma} \label{lemma_proof_optimize} 
	For a query-level MOO problem with $d$ serial stages only, Algorithm~\ref{alg:optimize} guarantees to find a subset of stage-level Pareto optimal points.
\end{lemma}

In proving Lemma \ref{lemma_proof_optimize}, we observe that Algorithm~\ref{alg:optimize} is essentially a Weighted Sum procedure over Functions (WSF). Indeed we will prove the following two Propositions: 1) each solution returned by WSF is Pareto optimal; 2) the solution returned by the function \textit{optimize}  is equivalent to the solution returned by WSF. Then it follows that the solution returned by Algorithm~\ref{alg:optimize} is Pareto optimal.

To introduce WSF, we first introduce the indicator function $x_{ij}$, $i \in [1, ..., d], j \in [1, ..., p_i]$, to indicate that the $j$-th solution in $i$-th stage is selected to contribute to the query-level solution. $\sum_{j=1}^{p_i} x_{ij} = 1$ means that only one solution is selected for each stage. Then $x = [x_{1j_1}, ... x_{dj_d}]$ represents the 0/1 selection for all $d$ serial stages to construct a query-level solution.

So for the $v$-th objective, its query-level value could be represented as the function $H$ applied to $x$: 
\begin{equation}
    \begin{aligned}
    & F_v = H_v (x) = \sum_{i=1}^{d} \sum_{j=1}^{p_i} x_{ij} * f_{ijv}, \\
    & \quad where \sum_{j=1}^{p_i} x_{ij} = 1, i \in [1, ..., d], j \in [1, ..., p_i], v \in [1, ... k]
    \end{aligned}
\end{equation}

Now we introduce the Weighted Sum over Functions (WSF) as: 

\begin{align}
& \arg\!\min_{x} (\sum_{v=1}^{k} w_v * H_v(x)) \\
\mbox{s.t.} & \;\; \sum_{v=1}^{v} w_v = 1 
\end{align}


Next, we prove for Lemma \ref{lemma_proof_optimize}. As stated before, It is done in two steps. 

\begin{proposition}
	The solution constructed using $x$ returned by WSF is Pareto optimal.
\end{proposition}
% \textbf{proposition 1.1: The optimal solution returned by WSF is Pareto optimal}:

\begin{proof}
	~\\
	\indent Assume that $x^*$ (corresponding to $[F_1^*, ..., F_{k}^*]$ ) is the solution of WSF.
	Suppose that an existing solution $[F_1^{'}, ..., F_{k}^{'}]$ (corresponding to $x^{'}$)  dominates $[F_1^*, ..., F_{k}^*]$. This means that $\sum_{v=1}^{k} w_v * H_v({x^{'}})$ is less than that of $x^*$. \par
	This contradicts that  $x^*$ is the solution of WSF. So there is no $[F_1^{'}, ..., F_{k}^{'}]$ dominating $[F_1^*, ..., F_{k}^*]$. Thus, $[F_1^*, ..., F_{k}^*]$ is Pareto optimal.
\end{proof}

\begin{proposition}
	The optimal solution returned by the \textit{optimize} in Algorithm \ref{alg:optimize} is equivalent to the solution constructed using $x$ returned by WSF.
\end{proposition}

\begin{proof}
	~\\
	\indent Suppose $x^{'}$ is returned by WSF. The corresponding query-level solution is $[F_1^{'}, ..., F_{k}^{'}]$
	\begin{equation}
	\begin{split}
	x^{'} & = \arg\!\min(\sum_{v=1}^{k} w_v * H_v(x))\\
	& = \arg\!\min(\sum_{v=1}^{k} w_v * (\sum_{i=1}^{d} \sum_{j=1}^{p_i} x_{ij} * f_{ijv}))\\
	& = \arg\!\min(\sum_{i=1}^{d} (\sum_{v=1}^{k} \sum_{j=1}^{p_i} (w_v * f_{ijv}) * x_{ij}))
	\end{split}
	\end{equation}
	
	For the solution $[F_1^{''}, ..., F_{k}^{''}]$ returned by the Algorithm \ref{alg:optimize}, $x^{''}$ represents the corresponding selection. It is achieved by minimizing the following formula:
	
	\begin{equation}
	\begin{split}
	& \sum_{i=1}^{d} (WS_{ij} | j\in[1, p_i])\\
	& = \sum_{i=1}^{d} (\sum_{v=1}^{k} w_v * f_{ijv} | j\in[1, p_i])\\
	& = \sum_{i=1}^{d} (\sum_{v=1}^{k} \sum_{j=1}^{p_i}
	(w_v * f_{ijv}) * x_{ij})\\
	\end{split}
	\end{equation} 
	where $WS_{ij} = \sum_{v=1}^{k} w_v * f_{ijv}$. 
	
	So, we have:
	\begin{equation}
	\begin{split}
	x^{''} & = \arg\!\min(\sum_{i=1}^{d} (\sum_{v=1}^{k} \sum_{j=1}^{p_i} (w_v * f_{ijv}) * x_{ij}))
	\end{split}
	\end{equation}
	\noindent 
	 Since they are of the same form and achieve min at the same time, so we have $[F_1^{'}, ..., F_{k}^{'}] = [F_1^{''}, ..., F_{k}^{''}]$
	
\end{proof}
 
With these two propositions, we finish the proof of Lemma \ref{lemma_proof_optimize}.

Assume there is a query with $B$ branches to be merged further. Operation 2) includes optimizing each serial branch and merging these branches. For optimizing each serial branch, it is equivalent to the Algorithm \ref{alg:optimize}. After optimizing, there are $B$ Pareto sets, where the latency of the query is the maximum over $B$ branches, and the cost is the sum.


If the one objective is calculated as the maximum over two branch results, the WSF is defined as:

So for the $v$-th objective, its query-level value could be represented as the function $H$ applied to $x$: 
\begin{equation}
    \begin{aligned}
    & F_v = H_v (x) = \max (\sum_{j=1}^{p_i} x_{ij} * f_{ijv} | i \in [1, ..., d])\\
    & \quad where \sum_{j=1}^{p_i} x_{ij} = 1, i \in [1, ..., d], j \in [1, ..., p_i], v \in [1, ... k]
    \end{aligned}
\end{equation}

\indent Suppose $x^{'}$ is returned by WSF. The corresponding query-level solution is $[F_1^{'}, ..., F_{k}^{'}]$
	\begin{equation}
	\begin{split}
	x^{'} & = \arg\!\min(\sum_{v=1}^{k} w_v * H_v(x))\\
	& = \arg\!\min(\sum_{v=1}^{k} w_v * (\max (\sum_{j=1}^{p_i} x_{ij} * f_{ijv}|i=[1,d])))
	\end{split}
	\end{equation}
	
	For the solution $[F_1^{''}, ..., F_{k}^{''}]$ returned by the Algorithm \ref{alg:optimize}, $x^{''}$ represents the corresponding selection. It is achieved by minimizing the following formula:
	
	\begin{equation}
	\begin{split}
	& \max (WS_{ij} | i \in [1,...,d], j\in[1, p_i])\\
	& = \max (\sum_{v=1}^{k} w_v * f_{ijv} | i \in [1,...,d], j\in[1, p_i])\\
	& = \max (\sum_{v=1}^{k} \sum_{j=1}^{p_i}
	(w_v * f_{ijv}) * x_{ij} | i \in [1,...,d])
	\end{split}
	\end{equation} 
	where $WS_{ij} = \sum_{v=1}^{k} w_v * f_{ijv}$. 
	
	So, we have:
	\begin{equation}
	\begin{split}
	x^{''} & = \arg\!\min(\max (\sum_{v=1}^{k} \sum_{j=1}^{p_i}
	(w_v * f_{ijv}) * x_{ij} | i \in [1,d]))
	\end{split}
	\end{equation}
	\noindent 
	 Since they are in different form, so we have $[F_1^{'}, ..., F_{k}^{'}] \neq [F_1^{''}, ..., F_{k}^{''}]$

\todo{what about objectives with a mixture of sum and max?
if there is only one objective with max, it keeps the optimality?---NO!}

Suppose there are $k_1$ objective to be summed and $k_2$ objectives to be maximized, its query-level value could be represented as the function $H$ applied to $x$: 
\begin{equation}
    \begin{aligned}
    & F_v = H_v (x) = \sum_{i=1}^{d} \sum_{j=1}^{p_i} x_{ij} * f_{ijs} + \max (\sum_{j=1}^{p_i} x_{ij} * f_{ijm} | i \in [1, ..., d])\\
    & \quad where \sum_{j=1}^{p_i} x_{ij} = 1, i \in [1, ..., d], j \in [1, ..., p_i] \\
    & \quad s \in [1, ... k_1], m \in [k_1+1, ... k_1 + k_2]
    \end{aligned}
\end{equation}

Since the two parts have the same variable $x_{ij}$, it cannot be splitted to optimize independently as shown in Algorithm \ref{alg:optimize}.

\begin{lemma} \label{lemma_proof_merge} 
	For a query-level MOO problem with $B$ branches and one exit stage, where each branch is composed of one or multiple serial stages, Algorithm~\ref{alg:merge_branches} guarantees to find a subset of query-level Pareto optimal points.
\end{lemma}

The proof is the same as that in \textit{raa\_path}


==> checkpoint-231115/Qi_initial_optimizer/query_moo_problem_statement.tex <==
\section{Problem Statement}

A Spark physical plan is represented as a Directed Acyclic Graph (DAG) of stages. Different stages are able to take different parameters, which decide the query performance and resource consumption.

Our project aims to tune Spark parameters for queries in Spark while meeting multiple performance requirements from users (e.g. query-level latency, cost, etc.). The Multi-Objective Optimization problem (MOO) arises when the multiple user performance objectives are conflicting. In our problem, we considered 12 knobs as shown in the following Table \ref{tab:spark-knobs}. All stages share the same values of $k1$ to $k8$ but can have different values for $s1$ to $s4$.

We have two levels of optimization problems to be solved. The first is the \textit{stage-level optimization problem}, which is to tune resource parameters for each stage to generate a Pareto set. Thus, from the stage level, users can select one from them based on their preference. However, different choices of stage-level Pareto solutions contribute to different query-level performances. \textit{Query-level optimization problem} is necessary to take the stage-level Pareto solutions as input and optimize for the query-level objectives.

The following query-level MOO considers a general case, which is able to optimize two or more objectives. So, some of the notations are different from the previous section, where the notations are shown in the Table \ref{tab:notation_query_moo}.

\begin{table}[t]
\ra{1.2}
\small
\caption{Notations in the query-level MOO}
\label{tab:notation_query_moo}
\centering
	\begin{tabular}{cl}\toprule
	Symbol & Description \\\midrule
%$S$ & the number of stages in $Q$ \\
$k$ & the number of objectives \\
$\bm{\theta_q}$ & the shared parameters among stages in $Q$  \\
$\bm{\theta_s}$ & the tunable parameters for the stage $s$ \\
$f^s$ & the Pareto set of the stage $s$ \\
$f_k^s$ & the $k$-th objective value of the stage $s$ \\
$\Phi_k$ & the predictive model from $\theta_s$ to the $k$-th stage-level objective, where $s=1,...,S$ \\
$F_k$ & the $k$-th objective value of the query $Q$ \\
$\Lambda_k$ & mapping from the stage value to the query by following the topological order of $Q$ \\
\bottomrule
	\end{tabular}
\end{table}

% \minip{Stage-level MOO.}
Assume there are $|S|$ stages. For each stage, we denote $k1$ to $k8$ as $\bm{\theta ^ q}$, and denote $s1$ to $s4$ as $\bm{\theta ^ s}$. $\bm{\theta ^ q}$ is the same for all stages in a query, while $\bm{\theta ^ s}$ could be different for different stages $s$. 

Then we have the Stage-level MOO Problem for stage $s$ defined as:

{\definition{\textbf{Stage-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:stage-mult_obj_opt_def}
		\arg \min_{\bm{\theta_q}, \bm{\theta_s}} &f^s(\bm{\theta_q}, \bm{\theta_s})=& {\left[
			\begin{array}{l}
			f_1^s(\bm{\theta_q}, \bm{\theta_s}) = \Phi_1(\bm{\theta_q}, \bm{\theta_s}) \\ 
			...\\
			f_k^s(\bm{\theta_q}, \bm{\theta_s}) = \Phi_k(\bm{\theta_q}, \bm{\theta_s})
			\end{array}
			\right]} %\\
%		\nonumber s.t. & &  {\begin{array}{l}
%			{f_i^s}^L \leq f_i^s(\bm{\theta_q}, \bm{\theta_s}) \leq {f_i^s}^U, \,\,\, i=1,...,k, s=1,...,S\\
%			\end{array}}
		\end{eqnarray}
}}
\noindent{where $\Phi_j$ is the predictive model from $\theta_s$ to the $j$-th stage-level objective}. The stage-level MOO problem can be solved by our existing work.

% \minip{Query-level MOO.}
For the query-level MOO problem, generally, there are $|\bm{\theta_q}| + S * |\bm{\theta_s}|$ parameters to be tuned.

Since the predictive model are built for each stage, the query-level value can be obtained in two cases: 1) building a query-level model by composing the stage-level models with the topological order, where the query-level value is obtained based on the query-level model; 2) fixing $\bm{\theta_q}$ and then tuning $\bm{\theta_s}$ of each stage to get its Pareto sets, where the query-level value is calculated based on the Pareto solutions of all stages.

The parameter space of the first case includes $|\bm{\theta_q}| + S * |\bm{\theta_s}|$ parameters, which is much larger than that of the second case ($|\bm{\theta_s}|$). Moreover, for stages, only Pareto optimal solutions contribute to the final Pareto optimal query-level solutions. Theoretically, if one query-level Pareto optimal solution includes any dominated stage-level solution (e.g. $r_1$), it means there is at least another non-dominated stage-level value (e.g. $r_1'$) to reduce the objective value (e.g. cost) further. It is contradictory to the statement that this query-level solution is Pareto optimal. Thus, it is impossible to include a dominated solution in any stage.


We have the general Query-level MOO Problem defined as:

{\definition{\textbf{General Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:general_query-mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})=& {\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Psi_1(\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}}) \\ 
			...\\
			F_k(\bm{\theta}) = \Psi_k(\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}})
			\end{array}
			\right]} %\\
%		\nonumber s.t. & &  {\begin{array}{l}
%			{F_i}^L \leq F_i(\bm{\theta}) \leq {F_i}^U, \,\,\, i=1,...,k\\
%			\end{array}}
		\end{eqnarray}
}}

\noindent{where $\theta = [\bm{\theta_q},\bm{\theta^1},...,\bm{\theta^{|S|}}]$ is parameters for all stages, $\Psi_j$ is the query-level model composed by the $S$ stage-level predictive models by following the DAG topology of the query.}
%to get the query-level objective values by following the topological order.}.

%\todo{While, the parameter space is decided by the number of stages. the query-level objective values are obtained after composing the $S$ stage-level predictive models together into the DAG. It is trivial/non-trivial to compose the stage-level into the query-level? After the composition, whether it will be slower to return predictions than the stage-level model? if so, how much it will increase the time complexity?}

\todo{
So, we approximate it to tune all stages in advance under the assumption of the invariant machine system state. The intuition is to find a decent $\bm{\theta_q}$ first, and tune $\bm{\theta_s}$ for each stage, so that we can get Pareto solutions for all stages in advance, and calculate the query-level values based on these stage-level values by following the DAG topology. }

\todo{
It can be easily proved that only the Pareto optimal stage-level solutions contribute to the query-level Pareto optimal solutions. Suppose that one query-level Pareto optimal solution $\bm{r}$ includes a dominated stage-level solution $\bm{s}$. It means there exists at least one query-level solution $\bm{r'}$ could include a stage-level solution $\bm{s'}$ dominating $\bm{s}$ with lower stage-level values. So that $\bm{r'}$ dominates $\bm{r}$, which contradicts that $\bm{r}$ is Pareto optimal. Thus, it is impossible that the final query-level Pareto optimal solution includes a dominated stage-level solution.
}

Thus, We have the Query-level MOO Problem defined as:

{\definition{\textbf{Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:query_mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})=& {\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Lambda_1(f_1^1(\bm{\theta_q},\bm{\theta^1}),...,f_1^{|S|}(\bm{\theta_q},\bm{\theta_{|S|}})) \\ 
			...\\
			F_k(\bm{\theta}) = \Lambda_k(f_k^1(\bm{\theta_q},\bm{\theta^1}),...,f_k^{|S|}(\bm{\theta_q},\bm{\theta_{|S|}})
			\end{array}
			\right]} %\\
%		\nonumber s.t. & &  {\begin{array}{l}
%			{F_i}^L \leq F_i(\bm{\theta}) \leq {F_i}^U, \,\,\, i=1,...,k\\
%			\end{array}}
		\end{eqnarray}
}}
\noindent{where $\theta = [\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_s}]$ is resource parameters for all stages, $\Lambda_j$ is the general function mapping from the stage-level Pareto solutions of all stages $f_j^1(\theta_1), ..., f_j^S(\theta_s)$ 
%$\{f_j^i(\theta_i) | i=1,...,|S|\}$
to the $j$-th query-level objective. This function mapping follows the calculation of the topological order of DAG}.

%\noindent{where $\theta = [\bm{\theta_q},\bm{\theta^1},...,\bm{\theta_s}]$ is resource parameters for all stages, $\Lambda_j$ is the general function mapping from the stage-level Pareto solutions of all stages $f_j^1(\theta^1), ..., f_j^S(\theta_s)$ to the $j$-th query-level objective. This function mapping follows the calculation of the topological order of DAG}.
%>>>>>>> Stashed changes

\cut{
For the corresponding MOO algorithms, the \textit{stage-level optimization problem} could be solved by our previous work in the ICDE paper. The following section will show the details of the MOO algorithm design for the \textit{query-level optimization problem}.
}

\begin{algorithm}[t]
	\caption{Query-level MOO}
	\label{alg:divided_and_conquer}
	\small
	\begin{algorithmic}[1]  
		\REQUIRE {$Q, \Phi_i, t$, $\forall i\in [1,k]$}.
        \STATE $\bm{\theta_q}=[], \bm{\theta}=[], \bm{f}=[]$
        \STATE \% {\textit{Step 1: get Pareto solutions for all stages}}
		\FOR {$s$ \textbf{in} $\bm{S}$}
            \STATE ${\bm{f}^s}$, ${\bm{\theta}}$ = stage\_moo(t, $\Phi$)
            \STATE $\bm{\theta_q}$.append(${\bm{\theta_q}}$)
        \ENDFOR
        \STATE \% {\textit{Step 2: union all $\theta_q$ candidates}}
        \STATE q\_set = set($\bm{\theta_q}$)
        \STATE \% {\textit{Step 3: tune $\bm{\theta_s}$ for each $\theta_q$}}
        \FOR {$q$ \textbf{in} q\_set}
            \STATE ${\bm{f}^s}$, ${\bm{\theta_s}}$ = fine\_tune(t, $\Phi$, $q$)
            \STATE $\bm{\theta}$.append($[q, \bm{\theta_s}]$), $\bm{f}$.append(${\bm{f}^s}$)
        \ENDFOR
        \STATE $\bm{F},\bm{\theta} = filter\_dominated(\Lambda(\bm{f}, \bm{\theta}))$
        \RETURN $\bm{F}$, $\bm{\theta}$
	\end{algorithmic}
\end{algorithm}

\todo{
The above definition is able to be solved in a "divided-and-conquer" manner. First, by tuning $\bm{\theta}$ for each stage, we can get a Pareto set for each stage. Thus, each stage could have multiple $\bm{\theta_q}$ candidates based on the tuned $\bm{\theta}$. After that, we union the $\bm{\theta_q}$ candidates of all stages together. In the query-level MOO problem, $\bm{\theta_q}$ is shared among all stages and $\bm{\theta_s}$ is tunable for each stage. To compare the performance of all $\bm{\theta_q}$ candidates, by fixing each $\bm{\theta_q}$, we continue to tune $\bm{\theta_s}$, and finally keep the configurations $\bm{\theta}$ which contribute to the query-level Pareto solutions as the optimal.
}

\todo{
The stage-level Pareto solutions could possibly following 3 rules.
First, as $\bm{\theta_q}$ is mainly related to the resource settings (e.g. k1, k2, k3 knobs), more resources allocated, lower latency will be.
Second, after fixing $\bm{\theta_q}$, the total resources of the query is fixed, where resources are shared among all stages. In this case, by tuning $\bm{\theta_s}$, the cost is linear to the latency. We can assume the cost follows the rule of $cost = q * latency$, where $q$ indicates the number of resources. A higher value means more resources.
Third, since $\bm{\theta_s}$ also affect the latency prediction, during tuning $\bm{\theta_s}$, the latency may fluctuate.
}

\todo{
The key problem of the above proposal is to make sure the $\bm{\theta}$ (with $\bm{\theta_q}$ candidates included) guarantee to contribute to the query-level Pareto optimal solution. }






==> checkpoint-231115/Qi_initial_optimizer/stage_level_tuning.tex <==
\section{Stage-level tuning}

A Spark physical plan is represented as a Directed Acyclic Graph (DAG) of stages. Different stages are able to take different parameters, which decide the query performance and resource consumption.

Our project aims to tune Spark parameters for queries in Spark while meeting multiple performance requirements from users (e.g. query-level latency, cost, etc.). The Multi-Objective Optimization problem (MOO) arises when the multiple user performance objectives are conflicting. In our problem, we considered 12 knobs as shown in the following Table \ref{tab:spark-knobs}. All stages share the same values of $k1$ to $k8$ but can have different values for $s1$ to $s4$.

The following query-level MOO considers a general case, which is able to optimize two or more objectives. So, some of the notations are different from the previous section, where the notations are shown in the Table \ref{tab:notation_query_moo}.

\begin{table}[t]
\ra{1.2}
\small
\caption{Notations in the query-level MOO}
\label{tab:notation_query_moo}
\centering
	\begin{tabular}{cl}\toprule
	Symbol & Description \\\midrule
%$S$ & the number of stages in $Q$ \\
$k$ & the number of objectives \\
$\bm{\theta_q}$ & the shared parameters among stages in $Q$  \\
$\bm{\theta_s}$ & the tunable parameters for the stage $s$ \\
$f^s$ & the Pareto set of the stage $s$ \\
$f_k^s$ & the $k$-th objective value of the stage $s$ \\
$\Phi_k$ & the predictive model from $\theta_s$ to the $k$-th stage-level objective, where $s=1,...,S$ \\
$F_k$ & the $k$-th objective value of the query $Q$ \\
$\Lambda_k$ & mapping from the stage value to the query by following the topological order of $Q$ \\
\bottomrule
	\end{tabular}
\end{table}

\subsection{Problem statement}

For the query-level MOO problem, generally, there are $|\bm{\theta_q}| + S * |\bm{\theta_s}|$ parameters to be tuned.

Since the predictive model are built for each stage, the query-level value can be obtained in two cases: 1) building a query-level model by composing the stage-level models with the topological order, where the query-level value is obtained based on the query-level model; 2) tuning $\bm{\theta}$ for each stage while maintaining the optimality in the query-level, where the query-level value is calculated based on the stage-level Pareto solutions, and the optimality means there is no other solutions could dominate it.

%The parameter space of the first case includes $|\bm{\theta_q}| + S * |\bm{\theta_s}|$ parameters, which is much larger than that of the second case ($|\bm{\theta_s}|$). Moreover, for stages, only Pareto optimal solutions contribute to the final Pareto optimal query-level solutions. Theoretically, if one query-level Pareto optimal solution includes any dominated stage-level solution (e.g. $r_1$), it means there is at least another non-dominated stage-level value (e.g. $r_1'$) to reduce the objective value (e.g. cost) further. It is contradictory to the statement that this query-level solution is Pareto optimal. Thus, it is impossible to include a dominated solution in any stage.


The parameter space of the first case includes $|\bm{\theta_q}| + |S| * |\bm{\theta_s}|$ parameters. And we have the general Query-level MOO Problem defined as:

{\definition{\textbf{General Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:1_general_query_mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})=& {\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Psi_1(\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}}) \\ 
			...\\
			F_k(\bm{\theta}) = \Psi_k(\bm{\theta_q},\bm{\theta_1},...,\bm{\theta_{|S|}})
			\end{array}
			\right]} %\\
%		\nonumber s.t. & &  {\begin{array}{l}
%			{F_i}^L \leq F_i(\bm{\theta}) \leq {F_i}^U, \,\,\, i=1,...,k\\
%			\end{array}}
		\end{eqnarray}
}}

\noindent{where $\theta = [\bm{\theta_q},\bm{\theta^1},...,\bm{\theta^{|S|}}]$ is parameters for all stages, $\Psi_j$ is the query-level model composed by the $S$ stage-level predictive models by following the DAG topology of the query.}

In the second case, we tune $\bm{\theta}$ for each stage, where the Query-level MOO problem is defined as: 

{\definition{\textbf{Query-level Multi-Objective Optimization (MOO).}
		\begin{eqnarray}
		\label{eq:sep_query_mult_obj_opt_def}
		\arg \min_{\bm{\theta}} &F(\bm{\theta})=& {\left[
			\begin{array}{l}
			F_1(\bm{\theta}) = \Lambda_1(\Phi_1(\bm{\theta^1}),...,\Phi_{|S|}(\bm{\theta^{|S|}})) \\ 
			...\\
			F_k(\bm{\theta}) = \Lambda_k(\Phi_1(\bm{\theta^1}),...,\Phi_{|S|}(\bm{\theta^{|S|}}))
			\end{array}
			\right]} %\\
%		\nonumber s.t. & &  {\begin{array}{l}
%			{F_i}^L \leq F_i(\bm{\theta}) \leq {F_i}^U, \,\,\, i=1,...,k\\
%			\end{array}}
		\end{eqnarray}
}}

\noindent{where $\theta^s = [\bm{\theta_q},\bm{\theta_s}], s=1,..,|S|$ is parameters for the stage $s$, $\Phi_s$ is the predictive model of the stage $s$. $\lambda_j$ is the general function mapping from the stage-level values to the $j$-th query-level objective values, which follows the calculation of the topological order of DAG.}

From the view of the parameter space, definition \ref{eq:1_general_query_mult_obj_opt_def} takes $|\bm{\theta_q}| + |S| * |\bm{\theta_s}|$ parameters, while the second case (problem \ref{eq:sep_query_mult_obj_opt_def}) takes $|\bm{\theta_q}| + |\bm{\theta_s}|$ as it tunes each stage separately. While, the first problem is able to search the whole parameter space, so its optimal solution guarantees to be optimal in the query-level. The second problem searches the parameter space in the stage-level, it is hard to say whether the calculation over the DAG graph contributes to be optimal in the query-level. We need extra strategies or algorithms to guarantee.

\subsection{A simplified problem}

In the problem \ref{eq:sep_query_mult_obj_opt_def}, $\bm{\theta_q}$ includes 8 parameters, and $\bm{\theta_s}$ includes 4 parameters. The following takes a simplified example to show how to guarantee the optimality if both $\bm{\theta_q}$ and $\bm{\theta_s}$ only include one parameter. Still, $\bm{\theta_q}$ are shared among all stages, and $\bm{\theta_s}$ can be different for different stages. After fixing $\bm{\theta_q}$, the query-level latency is linear to the cost. The main purpose of this simplified example is to give an intuition on how this problem is able to be solved while maintaining the optimality in the query-level.

When the $\bm{\theta_q}$ is 1-dim, it means we can enumerate all the $\bm{\theta_q}$ values as candidates, and then tune each $\bm{\theta_s}$ separately. In this way, it guarantees to explore a full set of solutions.

The Algorithm \ref{alg:1_dim_divided_and_conquer} is the corresponding Pseudo-code, where it assumes the $\bm{\theta_q}$ is the total number of cpu cores assigned to the query.

 \begin{algorithm}[t]
	\caption{Query-level MOO (1-dim $\theta_q$)}
	\label{alg:1_dim_divided_and_conquer}
	\small
	\begin{algorithmic}[1]  
		\REQUIRE {$Q, \Phi_i, t$, $\forall i\in [1,k], k2^l, k2^u, k3^l, k3^u$}.
        \STATE $\bm{\theta}=[], \bm{f}=[], \bm{\theta}\_list=[], \bm{f}\_list=[]$
        \STATE \% {\textit{Step 1: get all} $\bm{\theta_q}$}
		\STATE total\_cores\_set = get\_cores($k2^l, k2^u, k3^l, k3^u$)
        \STATE \% {\textit{Step 2: tune $\bm{\theta_s}$ for each $\theta_q$}}
        \FOR {$c$ \textbf{in} total\_cores\_set}
        	\STATE $\bm{\theta}.append$($c$)
        	\FOR {$s$ \textbf{in} $S$}
            	\STATE ${\bm{f}^s}$, ${\bm{\theta_s}}$ = fine\_tune(t, $\Phi$, $c$)
            	\STATE $\bm{\theta}.append$($\bm{\theta_s}$), $\bm{f}$.append(${\bm{f}^s}$)
            \ENDFOR
            \STATE $\bm{\theta}\_list.append$ ($\bm{\theta}$), $\bm{f}\_list.append$($\bm{f}$)
        \ENDFOR
        \STATE $\bm{F},\bm{\theta} = filter\_dominated(\Lambda(\bm{f}\_list, \bm{\theta}\_list))$
        \RETURN $\bm{F}$, $\bm{\theta}$
	\end{algorithmic}
\end{algorithm}


\subsubsection{Optimality analysis} \label{1-dim_optimality} ~

In the step 1, it obtains all candidates for $\bm{\theta_q}$, i.e. the total number of cpu cores for the query. Then, in step 2, it tunes $\bm{\theta_s}$ for each stage under each $\bm{\theta_q}$ candidate. Since the $\bm{\theta_q}$ is fixed, the $fine\_tune$ function solves a single-objective problem, which could return an optimal solution with lowest latency under one $\bm{\theta_q}$ candidate. 

\begin{proposition}
	The optimal solution returned by the Algorithm \ref{alg:1_dim_divided_and_conquer} is Pareto optimal in the query-level.
\end{proposition}

\begin{proof}
	~\\
	\indent Assume that $x^*$ (corresponding to $[F_1^*, ..., F_{k}^*]$ ) is the solution of Algorithm \ref{alg:1_dim_divided_and_conquer} under any arbitrary DAG graph, which is composed by the $\bm{\theta_q}$ and $\bm{\theta_s}, s=1,...,|S|$. For an arbitrary DAG, the query-level latency is calculated by following the topological order, and the query-level cost is the sum over all stage-level costs.\par
	Suppose that for the same DAG graph, an existing solution $[F_1^{'}, ..., F_{k}^{'}]$ (corresponding to $x^{'}$ with an arbitrary $\bm{\theta'_q}$)  dominates $[F_1^*, ..., F_{k}^*]$. 
	Firstly, Algorithm \ref{alg:1_dim_divided_and_conquer} explores all the values of $\bm{\theta_q}$, so this $\bm{\theta'_q}$ is definitely searched by Algorithm \ref{alg:1_dim_divided_and_conquer}. 
	Secondly, under any $\bm{\theta_q}$, for any stage, the function $fine\_tune$ guarantees to find the optimal solution with the lowest latency and cost. 
	Thirdly, the query-level cost is the sum over all stages, if $[F_1^{'}, ..., F_{k}^{'}]$ dominates $[F_1^*, ..., F_{k}^*]$, it means that there is at least one stage achieves lower cost than that of $x^*$, which is impossible due to the function $fine\_tune$.\par
 So there is no $[F_1^{'}, ..., F_{k}^{'}]$ dominating $[F_1^*, ..., F_{k}^*]$. Thus, $[F_1^*, ..., F_{k}^*]$ is Pareto optimal.
\end{proof}

\subsubsection{Complexity analysis} ~

Assume there are $\gamma$ $\bm{\theta_q}$ candidates, $|S|$ stages and the complexity of the $fine\_tune$ function is $\lambda$. The total complexity is $O(\gamma * |S| * \lambda)$.

\subsection{Algorithm design}

In the simplified problem, the Algorithm \ref{alg:1_dim_divided_and_conquer} enumerates the $\bm{\theta_q}$ candidates as it decides the number of the query-level solutions. 

Similarly, in our problem, after fixing $k1, k2, k3$ knobs, the query-level latency and cost are linearly correlated. It means the searching space of $k1, k2, k3$ decides the number of the query-level solutions. If we can get a full set of the searching space of $k1, k2, k3$, it is possible to find all the query-level Pareto optimal solutions for the problem \ref{eq:sep_query_mult_obj_opt_def}.

As described before, for each stage, the parameter space is divided into the $\bm{\theta_q}$, which is shared among all stages; and $\bm{\theta_s}$ which could be different among different stages. 
Each $\bm{\theta_q}$ can be divided further into two groups, where one (including $\bm{x} = \{x_1, x_2, x_3\}=\{k1, k2, k3\}$) is related to the resource settings, and the other one is related to the non-SQL knobs ($\bm{y} = \{k4, k5, k6, k7, k8\}$). After fixing $\bm{x}$, the query-level latency and cost is linearly correlated. Since each $\bm{\theta_q}$ only includes one set of $\bm{x}$, in other words,
after $\bm{\theta_q}$ is fixed, tuning $\bm{\theta_s}$ is a single-objective optimization problem in query-level. Based on this property, we can reduce the $\bm{\theta_q}$ into a 1-dim parameter. This reduction problem could be represented as the following:


{\definition{\textbf{Fixing resources.}
		\begin{eqnarray}
		\label{eq:fix_resources}
		\arg \min_{\bm{x, y, \theta_1, ..., \theta_{|S|}}} &F(\bm{x, y, \theta_1, ..., \theta_{|S|}}) \\
		\nonumber s.t. & {\begin{array}{l}
			{x_1 * x_3  = C_1 }\\
			{x_2 * x_3  = C_2 }\\
			\end{array}}
		\end{eqnarray}
}}

This is a single-objective optimization problem, where the total number of memory size and cores are subject to a constant ($C_1$ and $C_2$). 

The pseudo-code is as shown in Algorithm \ref{alg:8_dim_divided_and_conquer}:

 \begin{algorithm}[t]
	\caption{Query-level MOO (8-dim $\theta_q$)}
	\label{alg:8_dim_divided_and_conquer}
	\small
	\begin{algorithmic}[1]  
		\REQUIRE {$Q, \Phi_i, t$, $\forall i\in [1,k], k1^1, k1^u, k2^l, k2^u, k3^l, k3^u$}.
        \STATE $\bm{\theta}=[], \bm{f}=[], \bm{\theta}\_list=[], \bm{f}\_list=[]$
        \STATE \% {\textit{Step 1: get all resource candidates}}
		\STATE all\_candidates = enum($k1^1, k1^u, k2^l, k2^u, k3^l, k3^u$)
        \STATE \% {\textit{Step 2: tune $\bm{\theta}$ for each stage with the constraint of resource $c$}}
        \FOR {$c$ \textbf{in} all\_candidates}
        	\FOR {$s$ \textbf{in} $S$}
            	\STATE $\{ {\bm{f}^s} \}_Y$, $\{ {\bm{\theta}} \}_Y$ = fine\_tune(t, $\Phi$, $c$)
            	\STATE $\bm{\theta}.append$($
            	\{ {\bm{\theta}} \}_Y$), $\bm{f}$.append($\{ {\bm{f}^s} \}_Y$)
            \ENDFOR
            \STATE $\bm{\theta}\_list.append$ ($\bm{\theta}$), $\bm{f}\_list.append$($\bm{f}$)
        \ENDFOR
        \STATE $\bm{F},\bm{\theta} = filter\_dominated(\Lambda(\bm{f}\_list, \bm{\theta}\_list))$
        \RETURN $\bm{F}$, $\bm{\theta}$
	\end{algorithmic}
\end{algorithm}

Currently, line 3 enumerates all the combinations of resource knobs as the resource candidates. Under each resource candidate, for each stage, it tunes all the knobs including both $\bm{\theta_q}$ and $\bm{\theta_s}$. $\{ \}_Y$ indicates that the solutions with top $Y$ lowest latency are returned, where this top $Y$ includes the at least one intersection of $bm{y}$ knobs among all stages. Then, these solutions are kept to calculate the query-level solutions, where it guarantees to include the query-level Pareto optimal solutions.

\subsubsection{Optimality analysis} ~

The optimality in Algorithm \ref{alg:8_dim_divided_and_conquer} includes two parts: 1) enumerating over all resource knobs guarantee to find the full set of the query-level solutions; 2) under each resource constraint, within Top Y lowest latency values, the intersection of $\bm{y}$ among all stages must include the optimal query-level solution.


Since after fixing the resource knobs, tuning the rest knobs is a single-objective optimization problem, each resource knob combination at most results in one query-level optimal solution. So, the number of resource knob combination determines the upper bound the query-level Pareto optimal solutions.


\begin{proposition}
	Under each resource constraint $c$, by reserving top Y solutions with lowest latency, Algorithm \ref{alg:8_dim_divided_and_conquer} guarantees to return the optimal solution in the query-level.
\end{proposition}

\begin{proof}
	~\\
	\indent Assume that $x^*$ (corresponding to $[F_1^*, ..., F_{k}^*]$ ) is the solution of Algorithm \ref{alg:8_dim_divided_and_conquer} under an arbitrary DAG graph, which is composed by the $\bm{\theta_q}$ and $\bm{\theta_s}, s=1,...,|S|$. It is found within the top Y solution set constructed by the function $fine\_tune$. For an arbitrary DAG, the query-level latency is calculated by following the topological order, and the query-level cost is the sum over all stage-level costs.\par
	Suppose that for the same DAG graph, an existing solution $[F_1^{'}, ..., F_{k}^{'}]$ (corresponding to $x^{'}$ with the same resource constraint $c$ as $x^*$)  dominates $[F_1^*, ..., F_{k}^*]$ and not belongs to the top Y solution set. \par
	Under the same resource constraint, the top Y solution sets include the same resource knobs and at least one same set of $\bm{y}$ parameters among all stages. If $[F_1^{'}, ..., F_{k}^{'}]$ dominates $[F_1^*, ..., F_{k}^*]$, it means that, outside the top Y solution set, at least one stage achieves lower value than that in the top Y lowest values (returned by the function $fine\_tune$). It is impossible. \par
 So there is no $[F_1^{'}, ..., F_{k}^{'}]$ dominating $[F_1^*, ..., F_{k}^*]$. Thus, $[F_1^*, ..., F_{k}^*]$ is Pareto optimal.
	
\end{proof}

\subsubsection{Complexity analysis} ~

Assume there are $R$ resource knobs (each with maximum $V$ values), $\gamma$ resource candidates, $|S|$ stages and the complexity of the $fine\_tune$ function is $\lambda$. 

Line 3 takes $O(R^V)$.

The function $fine\_tune$ has already takes the top Y values into the consideration, 
so the total complexity is $O(R^V) + O(\gamma * |S| * \lambda)$.

\todo{how to efficiently determine resource candidates and top Y?}

==> checkpoint-231115/intro.tex <==
\section{Introduction}

% Formula
% application background
% the problem
% challenges wrt SOTA
% our big ideas 
% our contributions (including the results)


% Challenges in Spark (harder to model compared to other big data analytics systems)
Despite extensive research on modeling and optimizing queries in big data analytics systems~\cite{maxcompute, scope-vldb12, cleo-sigmod20, RO-alibaba}, the distinctive design of Spark SQL and its new default feature {\it Adaptive Query Execution (AQE)} presents additional complexities that make these problems more challenging. 

% multi-granularity control
Firstly, the configuration parameters in Spark could influence the execution of Spark SQL at different levels of granularity. 
The general Spark parameters are set at the application level and remain fixed after creating the Spark context. 
However, the SQL module introduces additional runtime parameters that can be adjustable when some runtime statistics are ready in the AQE framework.
Unfortunately, existing research~\cite{RAAL,lite-icde22,spark-moo-icde21,LOCAT-sigmod22} in Spark modeling and tuning primarily focuses on the application level, overlooking potential optimization opportunities at a more fine-grained level. 
For example, if we set configurations all in the application level, \todo{Figure}
shows that the optimal configuration for join\#1 is sub-optimal for join\#2, while we can make both optimal by controlling the runtime parameters at a finer-grained level.

\cut{
% mixed decision space
Secondly, configuration parameters in Spark SQL introduce a mixed decision space for optimization. 
Some runtime SQL parameters are plan-dependent and can alter the physical plan. For instance, the runtime parameters \textit{adaptive.autoBroadcastJoinThreshold} and \textit{adaptive.maxShuffledHashJoinLocalMapThreshold} influence the physical plan by deriving different join strategies. 
In contrast, all general Spark parameters and other SQL parameters like \textit{shuffle.partitions} are plan-independent and do not impact the physical plan.
As a result, the configuration tuning for Spark SQL involves deciding both the physical plan and other plan-independent parameters, which makes it more challenging compared to other approaches~\cite{cleo-sigmod20,adaptive-code-learning-spark-icde22,RO-alibaba,LOCAT-sigmod22} that focus solely on tuning plan-independent parameters.
}

% shared-resource environment
Secondly, the resource-to-stage mappings in Spark, while running an application, do not provide the same level of isolation as in other systems. Previous studies, such as those on MaxCompute~\cite{maxcompute} and SCOPE~\cite{scope-vldb12}, launched separate sets of executors for various stages, each utilizing different resource profiles. 
In contrast, Spark runs jobs in a resource-shared execution environment across parallel stages, resulting in tasks from different stages running on the same set of executors. 
While this design aligns with the desire for balanced input data in Spark, it introduces extra variance in the stage latency. For instance, in scenarios where parallel stages compete for resources, a multi-task stage might take longer to complete compared to running alone, as not all executors are exclusively allocated to the stage in such a resource-shared execution. 

% multi-objective space
\todo{Thirdly, the demand to get MOO}

In this study, we address the challenges of multi-granularity control\todo{, a mixed decision space?} and resource-shared execution in tuning configurations for Spark SQL, aiming to enhance query performance and resource utilization in a multi-objective optimization problem.

\todo{Our contributions include\begin{enumerate}
	\item a united modeling framework for query, subquery, and stage.
	\item the two-level optimization algorithm to support the multi-granularity control and achieve MOO
	\item Spark extension implementation and the evaluation results
\end{enumerate}}

\cut{
\highlight{introduces additional challenges in both modeling and optimization.}

%\todo{challenges in modeling, resource competing over parallel stages}
On the one hand, the latency of one stage could vary significantly due to the resource-shared execution in Spark, even with the same Spark configuration and machine system states. 
For example, suppose there is a stage doing a table scan with 20 tasks, and the executors have 20 cores.
When there are no parallel stages competing for resources, the 20 cores are assigned to the stage immediately so that the 20 tasks start running simultaneously.
However, when there is a competing stage (20 tasks) logically running ahead, our example stage would get cores dynamically from 1 (when the competing stage finishes the first task) to 20 (when the competing stage finishes running tasks). In this case, the example stage takes longer to finish all tasks than when there are no parallel stages.

%\todo{challenges in optimization, stage the shared configuration.}
On the other hand, configurations across different stages can not be set independently. With the resource-shared execution environment in Spark, only the SparkSQL-related parameters in the configuration can be set independently across different stages, and the remaining Spark parameters must be fixed across all the stages.
Therefore, adjusting the configuration for one stage could affect the optimality of other stages in the same Spark SQL, presenting additional challenges for optimization.
}




==> compile-time-opt-adaptive.tex <==
\rv{
\subsubsection{Adaptive Compile-time Optimization}

The compile-time optimization restricts itself to search only the query stage structure determined by the default configuration, which may not be the optimal structure and hence could be changed with AQE.
In addition, the solving time of compile-time optimization fails to adapt to longer running queries who could expect more solving time to achieve better performance gains.
Therefore, we propose the adaptive compile-time optimization to address the above concerns. Our approach, as shown in Algorithm~\ref{alg:adaptive_optimization}, adapts more searching space, in terms of more query stage structure exploration and more parameter searching within each HMOOC, to longer-running queries.


We begin with solving the query stage structure ($G_{default}$) derived from the default configuration. While solving $G_{default}$, we start a backend process to generate different query stage structures by varying $s_3$ and $s_4$ in $\thetabm_{sample}$, and push unseen query stage structures into a priority queue $\mathcal{G}$ with their predicted latency as the priority key. 
When $G_{default}$ is solved, we iteratively explore different query stage structures from $\mathcal{G}$ until the cumulative solving time exceeds the threshold or $\mathcal{G}$ is empty. 
In addition, we adapt the sampling rate for solving HMOOC provide larger parameter space exploration for longer-running queries within a HMOOC solving.

% We first vary $s_3$ and $s_4$ from $\thetabm_p$ to explore different subQ structures, denoted as $\mathcal{G}$, including (1) the default $s_3$ and $s_4$values, (2) 9 configurations from the Cartesian product of the min, mean, max values of $s_3$ and $s_4$, when other parameters are fixed.

% Then we iteratively explore different subQ structures until the cumulative solving time exceed the threshold, or $\mathcal{G}$ is empty, as shown in Algorithm~\ref{alg:adaptive_optimization}. By default, we set the threshold as the $5\%$ of the latency from the \po solution.

% \begin{algorithm}[t]
%     \caption{\rv{Adaptive Compile-time Optimization for Exploring Subquery (subQ) Structures}}
%     \label{alg:adaptive_optimization}
%     \small
%     \begin{algorithmic}[1]
%         \REQUIRE A set of subQ structures $\mathcal{G}$, the solving threshold rate $\alpha=0.05$.
%         \STATE $t_{cum} \gets 0$ % Initialize cumulative solving time
%         \STATE $lat^* \gets \infty$ % Initialize latency of the WUN PO solution
%         \STATE $\thetabm^* \gets \thetabm_{default}$
%         \WHILE{$(t_{cum} < lat^* \cdot \alpha) \AND (\neg \mathcal{G}.\text{is\_empty}())$}
%             \STATE $G \gets \mathcal{G}.\text{pop}()$ % Pop the next subquery from Q
%             \STATE $lat_{wun}, \thetabm_{wun}, dt \gets \text{HMOOC}(G)$ % Solve sq and get its latency and solving time
%             \IF{$lat_{wun} < lat^*$}
%                 \STATE $lat^* \gets lat_{wun}$ % Update the minimum latency
%                 \STATE $\thetabm^* \gets \thetabm_{wun}$ % Update the optimal configuration
%             \ENDIF
%             \STATE $t_{cum} \gets t_{cum} + dt$ % Update cumulative solving time
%         \ENDWHILE
%         \RETURN $\thetabm^*$ % Return the optimal thetabm
%     \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
    \caption{Adaptive Compile-time Optimization to Explore Query Stage Structures with Dynamic Generation}
    \label{alg:adaptive_optimization}
    \small
    \begin{algorithmic}[1]
        \REQUIRE The solving threshold rate $\alpha = 0.05$; Latency predictor $\Lambda: G \times \Theta \rightarrow \R$; Sample rate classifier $\Gamma: \R \rightarrow \{High, Low\}$; \\
        $t_0 = 1s$: minimum solving time; Default configuration $\thetabm_{default}$.
        \STATE $\{t_{cum}, lat^*, \thetabm^*, \mathcal{G}\} \gets \{0, \infty, \thetabm_{default}, \text{new priority queue}() \}$
        % \STATE $t_{cum} \gets 0$ % Initialize cumulative solving time
        %         , $lat^* \gets \infty$ % Initialize latency of the WUN PO solution
        %         , $\thetabm^* \gets \thetabm_{default}$ % Initialize the optimal configuration
        %         , $\mathcal{G} \gets \text{new priority queue}()$ % Initialize an empty priority queue
        \STATE $G_{default} \gets \text{Analyze}(\thetabm_{default})$ % Analyze the default configuration
        \STATE $\mathcal{G}.\text{push}(\Lambda(G_{default}, \thetabm_{default}), G_{default})$ % Push initial G with predicted latency
        \STATE Start a backend process: Generate for each sampled $\thetabm_{sample}$, and push unseen query stage structures $G_{\thetabm_{sample}}$ into $\mathcal{G}$ with its predicted latency $\Lambda(G_{\thetabm_{sample}}, \thetabm_{sample})$ as the priority key.
        \WHILE{$(t_{cum} < \max(lat^* \cdot \alpha, t_0)) \AND (\neg \mathcal{G}.\text{is\_empty}())$}
            \STATE $\hat{lat}, G \gets \mathcal{G}.\text{pop}()$ % Pop the next subquery with the highest priority (lowest latency)
            \STATE Sample rate $\gamma \gets \Gamma(\hat{lat})$
            \STATE $lat_{wun}, \thetabm_{wun}, dt \gets \text{HMOOC}(G, \gamma)$ % Solve G and get its latency, configuration, and solving time
            \IF{$lat_{wun} < lat^*$}
                \STATE $lat^* \gets lat_{wun}$ % Update the minimum latency
                , $\thetabm^* \gets \thetabm_{wun}$ % Update the optimal configuration
            \ENDIF
            \STATE $t_{cum} \gets t_{cum} + dt$ % Update cumulative solving time
        \ENDWHILE
        \RETURN $\thetabm^*$ % Return the optimal configuration
    \end{algorithmic}
\end{algorithm}


}


==> experiments/expt-q-tuning.tex <==
\subsection{Query-level Tuning Evaluation}

We define the realistic manual tuning strategy as follows. We pick 40 configurations that vary only in the resource-related knobs and vary only in the SQL-related knobs, respectively, and filter the non-dominated performances among the 80 configurations as the realistic performance upper bound in the objective space. 
In our example, the manual tuning costs $\approx 2$ weeks to run 22 representing TPCH queries in 80 configurations (each with three repeated runs).


\underline{Expt 5:} {\it Dominated space when the model is accurate.} 
We compare the recommendation quality, with respect to dominated space, of our model-based recommendation with the manual tuning and default configuration. To fact out the model uncertainty, we assume our model gives perfect latency prediction.

\underline{Expt 6:} {\it Dominated space when the model is inaccurate.}
We compare the dominated space in the realistic setting when the model is inaccurate.
In our model-based approach, we investigate the robust optimation method with static $\alpha$ choices $0,2,3$ and an adaptive one.


\underline{Expt 7:} {\it End-to-end comparison.}
We show the net benefit of our model-based approach against the manual tuning and the default setting (with AQE on), where we picked K queries that have not been manually tuned from each template. For manual-tuned configuration, we reuse the best configuration from the representative query in the same template.
\todo{run over test queries}



\cut{ % old results for Spark with AQE disabled. 
\begin{table*}[t] %local
\ra{1}
\small
\addtolength{\tabcolsep}{2pt}
\newrobustcmd{\B}{\bfseries}
\begin{tabular}{lccccccccc}
\toprule
Q   & default & res & sql & rb(-3) & rb(-2) & rb(0) & rb(+2) & rb(+3) & vc \\ % ws
\midrule                 
q1&   10\%&   72\%&   14\%&   86\%&   90\%&   90\%&   91\%&   91\%&   72\%    \\
q2&   7\%&    15\%&   72\%&   95\%&   95\%&   98\%&   96\%&   96\%&   97\%    \\
q3&   4\%&    41\%&   55\%&   78\%&   77\%&   87\%&   88\%&   90\%&   53\%    \\
q4&   27\%&   75\%&   49\%&   70\%&   67\%&   80\%&   73\%&   73\%&   50\%    \\
q5&   12\%&   32\%&   54\%&   90\%&   90\%&   80\%&   75\%&   71\%&   69\%    \\
q6&   33\%&   69\%&   41\%&   39\%&   67\%&   75\%&   78\%&   75\%&   74\%    \\
q7&   23\%&   28\%&   74\%&   92\%&   95\%&   96\%&   94\%&   94\%&   94\%    \\
q8&  27\%&   50\%&   82\%&   83\%&   82\%&   77\%&   82\%&   84\%&   76\%    \\
q9&  0\%&    19\%&   60\%&   91\%&   91\%&   92\%&   94\%&   94\%&   88\%    \\
q10&  17\%&   42\%&   64\%&   71\%&   74\%&   81\%&   79\%&   81\%&   71\%    \\
q11&  11\%&   19\%&   50\%&   73\%&   82\%&   72\%&   76\%&   72\%&   74\%    \\
q12&  0\%&    37\%&   48\%&   80\%&   82\%&   81\%&   82\%&   82\%&   82\%    \\
q13&  45\%&   73\%&   57\%&   85\%&   84\%&   86\%&   84\%&   86\%&   85\%    \\
q14& 24\%&   52\%&   39\%&   5\%&    5\%&    5\%&    1\%&    1\%&    5\%     \\
q15&  26\%&   56\%&   48\%&   38\%&   59\%&   71\%&   79\%&   75\%&   83\%    \\
q16&  0\%&    2\%&    43\%&   84\%&   87\%&   89\%&   83\%&   83\%&   77\%    \\
q17&  45\%&   86\%&   46\%&   78\%&   81\%&   75\%&   74\%&   74\%&   69\%    \\
q18&  22\%&   63\%&   45\%&   95\%&   95\%&   91\%&   90\%&   84\%&   69\%    \\
q19&  24\%&   50\%&   48\%&   85\%&   85\%&   81\%&   82\%&   82\%&   80\%    \\
q20&  1\%&    3\%&    83\%&   95\%&   95\%&   99\%&   99\%&   99\%&   99\%    \\
q21&  15\%&   52\%&   23\%&   89\%&   89\%&   89\%&   90\%&   90\%&   81\%    \\
q22&  25\%&   59\%&   40\%&   53\%&   54\%&   44\%&   36\%&   55\%&   54\%    \\
AVG&    18.2\%& 45.2\%& 51.7\%& 75.2\%& 78.4\%& 79.0\%& 78.5\%& 78.6\%& 72.8\%\\
STD&    13.2\%& 23.1\%& 16.5\%& 22.2\%& 19.7\%& 19.8\%& 21.0\%& 19.7\%& 19.5\%\\
\bottomrule
\end{tabular}
\caption{Dominated Space in TPCH (AQE off)}
\label{tab:qtuning-po-aqe-off}
\end{table*}


\begin{table*}[t] %local
\ra{1}
\small
\addtolength{\tabcolsep}{2pt}
\newrobustcmd{\B}{\bfseries}
\begin{tabular}{lccccccccc}
\toprule
Q   & default & res & sql & rb(-3) & rb(-2) & rb(0) & rb(+2) & rb(+3) & vc \\ % ws
\midrule                 
q1 &   8\%&    71\%&   12\%&   80\%&   89\%&   88\%&   88\%&   88\%&   70\%    \\
q2 &   0\%&    48\%&   61\%&   92\%&   92\%&   87\%&   83\%&   83\%&   86\%    \\
q3 &   20\%&   40\%&   57\%&   83\%&   81\%&   87\%&   89\%&   92\%&   59\%    \\
q4 &   28\%&   76\%&   45\%&   65\%&   67\%&   79\%&   76\%&   76\%&   72\%    \\
q5 &   9\%&    30\%&   45\%&   92\%&   92\%&   72\%&   72\%&   70\%&   59\%    \\
q6 &   40\%&   75\%&   51\%&   21\%&   53\%&   73\%&   73\%&   71\%&   70\%    \\
q7 &   9\%&    20\%&   69\%&   91\%&   93\%&   94\%&   91\%&   91\%&   92\%    \\
q8 &  47\%&   68\%&   75\%&   78\%&   77\%&   72\%&   73\%&   73\%&   68\%    \\
q9 &  14\%&   29\%&   61\%&   97\%&   97\%&   95\%&   96\%&   96\%&   93\%    \\
q10 &  36\%&   68\%&   66\%&   67\%&   66\%&   74\%&   79\%&   80\%&   72\%    \\
q11 &  21\%&   36\%&   58\%&   63\%&   86\%&   62\%&   80\%&   72\%&   71\%    \\
q12 &  1\%&    47\%&   43\%&   76\%&   77\%&   75\%&   77\%&   76\%&   77\%    \\
q13 &  38\%&   69\%&   48\%&   81\%&   78\%&   79\%&   82\%&   84\%&   83\%    \\
q14 & 42\%&   78\%&   49\%&   3\%&    3\%&    6\%&    6\%&    3\%&    4\%     \\
q15 &  64\%&   92\%&   84\%&   28\%&   44\%&   51\%&   52\%&   52\%&   54\%    \\
q16 &  18\%&   31\%&   43\%&   65\%&   69\%&   72\%&   56\%&   56\%&   54\%    \\
q17 &  45\%&   84\%&   43\%&   68\%&   76\%&   80\%&   75\%&   75\%&   66\%    \\
q18 &  36\%&   82\%&   30\%&   94\%&   94\%&   86\%&   86\%&   86\%&   67\%    \\
q19 &  24\%&   50\%&   42\%&   77\%&   77\%&   74\%&   75\%&   75\%&   74\%    \\
q20 &  6\%&    17\%&   50\%&   73\%&   73\%&   87\%&   87\%&   87\%&   84\%    \\
q21 &  20\%&   52\%&   30\%&   88\%&   89\%&   90\%&   90\%&   90\%&   85\%    \\
q22 &  29\%&   67\%&   50\%&   69\%&   74\%&   68\%&   59\%&   68\%&   66\%    \\
AVG&    25.1\%& 55.9\%& 50.6\%& 70.4\%& 74.9\%& 75.0\%& 74.8\%& 74.8\%& 69.3\%\\
STD&    16.4\%& 21.9\%& 15.4\%& 23.8\%& 20.3\%& 18.3\%& 18.7\%& 19.0\%& 17.9\%\\
\bottomrule
\end{tabular}
\caption{Dominated Space in TPCH (AQE on)}
\label{tab:qtuning-po-aqe-on}
\end{table*}


\begin{table*}[t]
\ra{1}
\small
\addtolength{\tabcolsep}{2pt}
\newrobustcmd{\B}{\bfseries}
\begin{tabular}{lccccccccc}
\toprule
AQE   & default & res & sql & rb(-3) & rb(-2) & rb(0) & rb(+2) & rb(+3) & vc \\ % ws
\midrule                 
OFF      \\
ON       \\
\bottomrule
\end{tabular}
\caption{Dominated Space in TPCH (summary over 22 queries in TPCH)}
\label{tab:qtuning-po}
\end{table*}
}

==> experiments/expt-qs-tuning.tex <==
\subsection{QueryStage-level Tuning Evaluation}

\todo{Expt 8-10: similar as Expt 5-7}

==> response.tex <==
\begin{center}
    {\bf \uppercase{ \Large Response Letter for PVLDB Vol 17 Paper \#1785 {(\em Revision)}}}
    \end{center}
    
\noindent We thank all the reviewers for their constructive feedback. In this document, we summarize the revisions that we have performed based on reviewers' comments, followed by the revised manuscript, where the modified text is highlighted in \rv{magenta}.
    

%--------------------------------------------------------------------------------------------------------------------
\section*{Meta-Reviews}

\revheading{V1:} \revitem{Improved technical presentation (R1.D1, R1.D2, R1.D5, R2.W2, R2.W3, R2.W4, R2.D6, R4.D2)}

We have significantly improved the writing of our paper by addressing all of these  requests. Please see our detailed response to each reviewer below.

\revheading{V2:} \revitem{ New experiments or better explanation of the experiments (R1.D3, R1.D4, R1.D6, R2.W1, R4.D1)}

We have performed a major revision to add new experimental results to address all of the requests above. Please see our detailed response to each reviewer below. 

\input{response/R1}

\input{response/R2}

\input{response/R4}


==> response/R1.tex <==
\section*{Reviewer 1}

All of our references to the appendices refer to our tech report online: 
https://chenghao.pages.dev/papers/vldb24-lyu-tr.pdf~\cite{tech-report}

\revheading{R1.W1/D1:} \revitem{The proposed approach is complex involving a hybrid compile-time/runtime optimization method and modeling techniques. This complexity could pose implementation challenges in practice. Related to W1, even bringing seemingly simple solutions to a mature product at cloud scale is challenging. I would like to see more discussion around the practical aspects of integrating such a solution.}

To respond to the reviewer's comment, we added a paragraph at the beginning of Section 6 on the implementation details. We implemented different modules of our system as plugins into a Spark cluster. We further reported 1) the time overhead of collecting runtime statistics; 2) the time overhead of compile-time optimization; 3) the time overhead of runtime optimization; 4) model training time.  Overall, these overheads appear to be modest enough to permit future large-scale real-world  prototyping and deployment. 

%To respond to the reviewer's comment, we reported the four components and their corresponding overhead at the beginning of Section~\ref{sec:expt}. In particular, we design our components as different plugins into a Spark cluster, and hence can leverage the Spark's large-scale property to any cloud scale.
%This design makes our hybrid optimization an easy-to-use product for other Spark users.

% \chenghao{
%     In the experiment setup, bring the following information to make it clear.
%     \begin{enumerate}
%         \item the overhead to collect the traces needed for training \& optimization
%         \item the training/tuning overhead
%         \item the optimization overhead
%     \end{enumerate}
% }

\revheading{R1.W2/D2:} \revitem{The paper is quite dense to read. It would be good to provide more intuitive understanding early on before delving deeper. Related to W2, there are a lot of moving parts of the proposed solution primarily because the paper tries to address the optimization problem at a finer-granularity than prior work. This complexity might be mandated however it would be good to provide more intuitive understanding to the readers before jumping straight into the details.}

We thank the reviewer for the suggestion. We have significantly improved Section 3 to provide more intuitive understanding of the fine-grained parameter tuning problem and our overall approach, by leaving out  details to later sections. Please see the highlighted text in Section 3. 
In particular, 
\begin{itemize}
\item we improved the opening paragraphs of the subsections; 
\item we shortened Section 3.2 to highlight the benefits and complexity of fine-grained parameter tuning, by keeping the main message and a clear example in each paragraph; 
\item we rewrote Section 3.3.1 to give a more direct description of our compile-time/runtime optimization approach; 
\item we improved Section 3.3.2 to show a clear distinction between single-objective and multi-objective optimization, before delving into the mathematical definition. 
\end{itemize}


 %\todo{Section 3: 1) Intro: Expand the first paragraph to better explain what topics are covered. 2) Section 3.2 Fine-grained control has performance benefits, e.g., we can change the query plan. The writing is defensive and can be simplified: just keep the first sentence and go directly to Figure 3(a). Better write the sentence of 4.5G and explain that this is more shuffle than expected.  Next paragraph, we can drop the sentence "one may wonder". 3) Section 3.3 The opening sentence is incomplete and give more a complete overview.  4) Section 3.3.1 First sentence should be direct: we introduce two optimizers as shown in the red boxes of Figure 2. One is the compile time, the other is the runtime. 5) Section 3.3.2: First introduce multiple objectives. Then prior work does not work well. Then introduce the MOO definition. Finally the Spark definition.   }


\revheading{R1.W3/D3:} \revitem{The experimental evaluation did not give the readers a good sense of current limitations of the proposed approach i.e., where it fails and hence what could be some interesting future extensions to address those limitations. Related to W3, I would like to see additional experiments including cases where the proposed approach is either too slow or does not result in any improvement in the workload latency, for example. Plus a presentation of a few insights around such cases.}

We appreciate the reviewer's feedback and have added a new experiment, \underline{Expt 8}, in Section 6.3 to discuss the limitations of our proposed approach.
In particular, Figure~\ref{fig:all_tpch} and ~\ref{fig:all_tpcds} show the per-query latency using  \rt\ or the default configuration. 
Among the 22 TPC-H and 102  TPC-DS queries, \rt\ significantly outperforms the default for most of the queries,  while being similar (within 2s latency improvement) for three short-running queries. \rt\ loses to the default configuration only for one short-running query (\texttt{h14}), mainly due to the model error in predicting its latency. As we use WMAPE as the training loss to give more weight to long-running queries, short queries can have inaccurate predictions and hence experience a suboptimal query plan or insufficient resource allocation.
Future work could focus on improving latency prediction for short-running queries by developing specialized models or incorporating adaptive mechanisms based on a learned long-short query classifier. 

%We appreciate the reviewer's feedback and have conducted additional experiments in Expt \todo{9} to address the concerns regarding the limitations of our proposed approach. Figures~\ref{fig:all_tpch} and~\ref{fig:all_tpcds} demonstrate the per-query latency comparison between our proposed approach and the default configurations. Among 22 queries in TPC-H and 102 queries in TPC-DS, one short-running query (\texttt{h14}) performed worse than the default configuration, and three short-running queries (\texttt{h6}, \texttt{ds8}, \texttt{ds20}) showed performance similar to the default configuration, with a latency improvement within 2 seconds. The remaining queries significantly outperformed the default configuration. The primary limitation identified is the reduced accuracy in predicting the latency of short-running queries, due to the prioritization of long-running query prediction accuracy in the loss design of weighted mean absolute percentage error (WMAPE), which can result in suboptimal resource assignments or query plans for short-running queries. Future work could focus on improving latency prediction accuracy for short-running queries by developing specialized models or incorporating adaptive mechanisms based on a learned long-short query classifier. 


% \begin{enumerate}
%     \item
%     \chenghao{Explain why: (a) missing good structure (training error + more solving overhead); 
%     \item Point out the bad examples when we include three query plans. 
%     \item Perhaps in the appendix, currently only apply the shallow search over the parameters space, more details in how to address it in R2.D4; or (c) model accuracy?}
% \end{enumerate}


\revheading{R1.D4:} \revitem{Related to experiments, it appears 19 parameters were considered, how does the optimization approach scale with the number of parameters?}

\begin{figure}[t]
    \centering
    \includegraphics[width=.327\linewidth]{figs/parameters/fi-normalized-zoomin.pdf}
    \captionof{figure}{\small{Aggregated feature importance scores of the selected Spark parameters across four models}}
    \label{fig:rv-fis}
    % \begin{tabular}{lr}
    %     \subfigure[\small{Zoom out}]
    %     {\label{fig:fi-norm-origin}\includegraphics[width=.48\linewidth]{figs/parameters/fi-normalized-origin.pdf}}
    %     \hfill
    %     \subfigure[\small{Zoom in}]
    %     {\label{fig:fi-norm-origin}\includegraphics[width=.48\linewidth]{figs/parameters/fi-normalized-zoomin.pdf}}				
    % \end{tabular}
    % \caption{\small{Normalized feature importance scores of all parameters across four models}}
    % \label{figs:fi-norm}
\end{figure}

%To address the issue, we use our previous work~\cite{spark-moo-icde21} to form an important parameter set $\thetabm_c$, applying the LASSO-path feature selection approach (as used in Ottertune~\cite{VanAken:2017:ADM}) and integrating domain knowledge from Spark documentation.

We significantly extended our paper, including new techniques and new writing, to address the dimensionality of the parameter space. 
%Our changes include the following.
\begin{enumerate}
\item Initial feature selection: We first clarify that Spark has over 100 parameters and we selected 19 features as follows. (a) We keep query plan parameters $\thetabm_p$ and partition related parameters $\thetabm_s$, which can be replicated to have one copy for each query stage in our fine-grained tuning approach. (b) The dimensionality of the context parameter space ($\thetabm_c$) can reach up to hundreds~\cite{Locat_2022}. To address the issue, we apply the LASSO-path feature selection approach (as in our prior work~\cite{spark-moo-icde21} and in Ottertune~\cite{VanAken:2017:ADM}) and integrate domain knowledge from Spark documentation, resulting in a list of 8 context parameters. More details are in Appendix\techreportrv{~\ref{appendix:parameter-selection}}{~B.1}.
\item \underline{Feature importance score (FIS) based parameter filtering}: We conducted additional experiments to compute the feature importance scores (FIS) of the 19 parameters in our trained latency and data shuffle models. The FIS of a parameter here is defined to be the increase of the model error if the values of this parameter are randomly shuffled in the training set. Due to space limitations, we include one example in Figure~\ref{fig:rv-fis}, but leave other plots to \techreportrv{Figure~\ref{fig:fi-tpch-lat-all-parameters}-\ref{figs:fi-norm} in Appendix~\ref{appendix:fis-filtering}}{Figure 21-23 in Appendix B.3}. Our main observation is that the FIS values of the parameters, sorted in decreasing order,  follow a long tail distribution. The parameters at the tail, with a cumulative FIS less than 5\% in WMAPE, do not affect the model performance by much and hence can be filtered out. For instance, the threshold of 5\% cumulative FIS means an increment of at most 0.7\% in WMAPE for TPC-H and 1.2\% for TPC-DS in the subQ model.
% Our work applied FIS-based filtering of features, which are the features ranked at the long tail of the distribution with the cumulative loss not exceeding 5\% in WMAPE. 
% Given our current WMAPE results, the exceeding 5\% means 0.7\% more WMAPE in TPC-H and 1.2\% more WMAPE in TPC-DS for the subQ model.
\item \underline{Sampling with FIS-based parameter filtering}: Then we introduced three sampling methods that could leverage FIS-based selection: (a) random sampling with or without parameter filtering; (b) Latin hypercube sampling with or without parameter filtering; (c) adaptive grid search with inherent parameter filtering, as we described in the new paragraph starting with "Sampling methods" on Page 8, which is the last paragraph of Section~\ref{subsec:subq-tuning}.
\item \underline{New experimental results}: We added new results in Figure 11(b)-(c) to show performance metrics (hypervolume and solving time) of the above three sampling methods with parameter filtering. Among them, we report the adaptive grid search to be an overall winner, achieving the highest hypervolume among all FIS-based methods while keeping the solving time under 2s for most queries tested.
%\item \underline{Adaptive sampling}: We also conducted hyperparameter tuning of the sampling budget and further introduce a scheme that adjusts the sampling budget for the adaptive grid search method: If the predicted latency in default configuration is over 10s, we use the median sampling rate; otherwise, a low sampling rate, as introduced in \rv{Section~\ref{subsec:subq-tuning}}. Our analyses in \rv{\techreport{Appendix~\ref{appendix:adaptive-grid-search}}} show that further increasing the sampling rate does not improve performance but increases solving time, hence negatively impacting query performance.
% We provide the low, median, and high sampling rates for the adaptive grid search. When the predicted query latency  The sampling rate will   based on the predicted latency. We report the results in \todo{Table 6}.
% \item \todo{We further introduce the runtime adaptive scheme for the adaptive grid search. When the predicted latency is <10s, we use lower sampling rate, and medium sampling rate if over 10s. The High rate..., added after 2,3 in the paper.} \chenghao{descriptions in Sec5, and experiments in the tables, and report the numbers here: with the adaptiving scheme, we further improvement our performance.} 
% \item Re-organize
\end{enumerate}

% \todo{CL: add in the appendix to admit engineering work and say we pre-processed, full descriptions in the appendix.}


% \todo{
%     We have revised the writing in Section 5.1, Section 6.1, and Appendix include these new results.
% }

% In addition, while the SQL parameters $\thetabm_p$ and  $\thetabm_s$ have covered all SQL parameters, they are scaled to the number of query stages, hitting over 500 parameters in total. E.g., solving the TPC-DS query with 47 subQs, our algorithm deals with $47 \times (|\thetabm_p| + |\thetabm_s|) = 517$ parameters, increasing the complexity significantly. To address this issue, we apply the cross-over idea as described in section~\ref{subsec:hmooc}.
% \todo{Decide to keep it or drop it depending on our latest results. }


\revheading{R1.D5:} \revitem{Can the paper provide some citation or intuition around why the average runtime of MOO of 0.62-0.83 second acceptable in practice (I understand it's already much better than the other approaches but is it still acceptable or potentially too high?)}

We aim to set the solving time to be on the same scale (sub-seconds to seconds) as the VM/Container startup time in the cloud as pointed out by \cite{SharmaCST16,AgarwalJP15,LyuFSSD22}. This is also consistent with our prior experience in solving the resource optimization problem for AliCloud's serverless computing~\cite{LyuFSSD22}.

To better balance the query execution time and solving time, our revision further introduced a (simple) runtime adaptive scheme to adjust the sampling budget based on the predicted latency. This technique is introduced at the end of Section~\ref{subsec:subq-tuning} and used in our new end-to-end experiments in Section 6.3. Overall, it allows us to improve results a little further while keeping an average solving time of 0.7-0.8s. 

%In a nutshell, we conducted hyperparameter tuning to derive low, medium, and high values for the sampling budget. Our profiling results show that if the predicted latency using the default configuration is over 10s, it is better to use the median sampling rate; otherwise, a low sampling rate does not deteriorate the performance while saving time. 
%Our analyses in \rv{\techreport{Appendix~\ref{appendix:adaptive-grid-search}}} show that further increasing the sampling rate does not improve performance but increases solving time, hence negatively impacting query performance.

\revheading{R1.D6:} \revitem{Figure 10(g), the paper states that all queries for TPC-H and -DS are used but this figure shows only a subset (perhaps because of space constraints). What was the performance on other queries?}

We appreciate the reviewer's feedback. We have added \underline{Expt 8} in Section 6.3 to show the  performance of all TPC-H and TPC-DS queries. 

\revheading{R1.D7:} \revitem{Minor: I didn't understand why in Sec 6.1, experiments were numbered Expt 1, 2, 5,6, 7,9 and 10?}

We have fixed the numbering of experiments throughout Section 6.


==> response/R2.tex <==

\section*{Reviewer 2}

All of our references to the appendices refer to our tech report online: 
https://chenghao.pages.dev/papers/vldb24-lyu-tr.pdf~\cite{tech-report}

\revheading{R2.W1:} \revitem{The experiments only use the synthetic TPC benchmarks, which rely on very simple data distributions. It is not that difficult to correctly predict selectivity for uniformly distributed data. Hence it is essential that the experiments also include real data.}


We agree with the reviewer that real-world datasets would be valuable in the  experimental study. However, it is difficult to obtain a large real dataset within the revision window: in our effort to contact a cloud service provider for data sharing, we learned that any dataset involving query plans cannot be shared due to strict privacy constraints. 

Nonetheless, we managed to strengthen our experimental study by considering the data skew present in TPC-DS, which has a hybrid  domain of synthetic and real-world data~\cite{OthayothP06,PossNW07}.
We added a new experiment, \underline{Expt3} in Section 6.1, to understand the impact of data skew on our modeling techniques. Our major results are the following.  
\begin{enumerate}
	\item TPC-DS queries experience skewed data distributions in both base relations and intermediate RDDs.
	\item The correlations between model errors and skewness are close to 0 during runtime optimization. This indicates that once the skewness is captured by  runtime statistics, the model can work quite  well regardless of the skewness level. 
\end{enumerate}
 
%With runtime optimization, the cardinality estimation is less important because we use observed statistics during runtime. Therefore, the skewness may still affect the compile-time optimization, but not for the runtime optimization. Once the skewness is featuralized in the model, our models work well to a large extent as shown in Table~\ref{tab:skew-corr}.


% \chenghao{
% \begin{enumerate}
%     \item It is indeed a great idea to run over the real data. However, due to the security constraints, we are not able to get a large dataset within the revision window. 
%     \item TPCDS is designed with skew for the base relations, and we further observed more skews in the intermediate results (intermediate RDDs).
%     \item  With runtime optimization, the cardinality estimation is less important because we use observed statistics during runtime. It may still affect the compile-time optimization, but not for the runtime optimization.
%     \item Once the skewness is featuralized in the model, our models work well to a large extent. (Report how well our model is)
%     \item More details are discussed in \rv{Expt3}.
% \end{enumerate}
% % Unfortunately, due to the data security and privacy concerns, we are unable to use real data in our experiments.
% % However, since TPC-DS follows a hybrid approach of both synthetic and real world based data domain when generate data~\todo{cite}, we can further identify the skewness and analyze how it affected our experiments. 
% % Specifically, we observed two types of skewness in our TPC-DS.
% % First, TPC-DS tables have skewed data distributions. TPC-DS has 7 fact tables and 17 dimension tables. Fact tables have columns with highly skewed data, as we observed in \techreport{Appendix~\ref{appendix:skewness}}, particularly those involving foreign keys to dimension tables or columns storing metrics like sales and profits.
% % Second, we observed the skewness among the partitions in the intermediate RDD of each query stage during job execution.
% }

\revheading{R2.W2:} \revitem{The notion of a subquery is not well-defined in the paper. The authors seem to define it based on shuffle operations and data exchange operators in the physical query plan. However, a rewritten plan can have different shuffle requirements and hence different subqueries. And when both inputs of a join are already partitioned in the same way, then Spark automatically avoids shuffling, even for the shuffled hash join. This needs a more formal treatment in the paper.}


To respond to the reviewer's comment, we made a number of revisions to improve the paper.  
\begin{enumerate}
\item We rewrote Section 4.1 to clarify the distinction between runtime models and compile-time models for optimization.   
\begin{itemize} \item For runtime optimization, the Spark optimizer already offers the collapsed logical query plan (\collap) and query stages (QS) in the physical plan. Hence, we collect these data structures and build runtime \collap\ and QS models to enable fine-grained tuning. \item For compile-time optimization, however, Spark does not provide any data structures that would suit our goal of fine-grained tuning.  For this reason, we introduce the notion of {\em compile-time subquery} ({subQ}) to denote a group of logical operators that will correspond to a query stage (QS) when the logical plan is translated to a physical plan. We build a subQ model for fine-grained tuning at compile time.  The output of compile-time optimization is fed as a starting configuration to the runtime optimization, which will subsequently adjust parameters and  physical plans as AQE proceeds.  
    \end{itemize}	


\item 	As a further enhancement, we also introduced a compile-time technique that samples multiple physical plans for each query, as described in Section~\ref{subsec:multi-pqp-search}.
\item We added a new experiment, \underline{Expt 10} in Section 6.3, to show that by searching multiple query plans at compile time, several long-running queries with complex query structures have gained additional performance improvements.
\end{enumerate}



%We formalize the definition of compile-time subquery (subQ) in Section~\ref{subsec:ct-rt-models} and proposed the idea of multiple query plan parallel search in Section~\ref{subsec:multi-pqp-search} to mitigate the diversity of the query plan structures. Our additional \underline{Expt 10} shows that by searching multiple query plans at compile time in parallel, several long-running queries with complex query structures has gained additional performance improvements.


%\textbf{Compile-time model.} At compile time, Spark provides a logical query plan (LQP) and then a physical plan (PQP), but no any data structures that would suit our goal of fine-grained tuning.  Therefore, we introduce the notion of {\em compile-time subquery} ({subQ}) to denote a group of logical operators that will correspond to a query stage (QS) when the logical plan is translated to a physical plan. In other words, it is a sub-structure of the logical plan that is reversely mapped from a query stage in a physical plan. 


% \chenghao{
%     \begin{enumerate}
%         \item clarify the subquery definition.
%         \item explain with more details on how we  initially group a query plan into different subqueries 
%         \item give the idea of exploring more grouping strategies by using a diverse of configurations to derive subQueries.
%     \end{enumerate}
% }

\revheading{R2.W3:} \revitem{Similarly, the optimizer seems to treat subqueries in isolation when exploring optimal configurations for query plan and query stage parameters. In reality, earlier partitioning and implementation decisions affect the cost and running time of downstream stages. For instance, in isolation a downstream subquery plan P1 may look better than alternative P2, but if P2 can reuse a DataFrame that is still cached in memory, or can exploit a specific partitioning established upstream, it may be the better choice overall. The proposed optimizer partially takes this into account through collapsed LQP, but that only gives a "lookahead" of 1 stage. So the problem remains when optimizing across multiple downstream stages. Please discuss and clarify in the paper.}

 We clarify that our prior compile-time optimization did simplify the problem by only considering one fixed plan structure based on the default configuration, and treat the compile-time subqueries (subQs) independently to enable efficient algorithms. 
 
 During the revision, we improved our compile-time optimization with multi-query plan search, as described in Section~\ref{subsec:multi-pqp-search}. This technique is shown to provide additional performance improvements for several long-running queries with complex query structures. 
 
 The output of compile-time optimization is then fed as a starting configuration to the runtime optimization, which will subsequently adjust parameters and  physical plans as AQE proceeds. We clarified this in the first paragraph of Section~\ref{sec:runtime-opt}. More specifically, our AQE-based runtime optimization is a progressive procedure: upon the completion of each query stage, the reminder of the query, represented as a collapsed LQP, will be reoptimized. A downstream stage may be optimized multiple times as the collapsed LQP becomes updated. However, at the moment when all of its preceding stages finish execution, the stage gets the chance of being optimized (the last time) with all the latest statistics. Therefore, the characteristics of all the previously completed stages will be considered in this last optimization decision. 
 
% However, this does not mean our entire work treats them independently because our runtime optimizer will keep adapting the parameter choices as long as the query plan structures to changes during execution. 
 %In addition, the runtime optimization can ``lookahead" as many stages as necessary because it only triggers optimizations for the collapsed LQP (\collap) only when all the query stages rooted on it finish running.

% \chenghao{
%     \begin{enumerate}
%         \item Our compile-time optimization indeed fails to adapt to the change of subquery structures when starting with the initial query plan determined based on a default configuration. To address it, we proposed an adaptive search strategy to cover a larger range of subquery structures. \todo{We agree that our compile-time optimization considering one fixed query structre based on default configuren. The (qi's) algorithm treat subQs indepentently when to solve ...; this does not mean in our entire work we treat them indepenently. }        
%         \item Our runtime optimization can adapt the change of subquery structures by reoptimizing $\thetabm_p$ with observed cardinalities.
%         \item Runtime optimizer can only ``lookahead" as many as necessary -- it only triggers optimizations for collapsed LQP only when all non-dependent subQs rooted finish running.
%         \item (not sure adding mulitple plans...)

%     \end{enumerate}
% }

% \todo{Add adaptive search as an extension}

\revheading{R2.W4:} \revitem{It is not completely clear how Spark configuration optimization interacts with optimization of the distributed algorithm itself, for instance the number of partitions [1]. Please discuss this briefly in related work.}

%We thank the reviewer the suggestion. We added Li et al.~\cite{LiMRSY19} to Section~\ref{tab:related-work}. Specifically, Spark AQE is able to take those distributed algorithms as separate query optimization rules, and our framework can then include the hyperparameters in those algorithms in SQL parameters, and optimize those algorithms wrapped in rules within our framework. Due to the space limitation, we leave more details to \techreport{Appendix \todo{...}}

We thank the reviewer for the suggestion. We added Li et al.~\cite{LiMRSY19} to Section~\ref{tab:related-work}. Specifically, Spark AQE is able to take those distributed algorithms as separate query optimization rules, and our framework can then treat the hyperparameters of those algorithms as SQL parameters and optimize those algorithms by tuning their hyperparameters in compile-time/runtime optimization. Due to space limitations, we leave more details to Appendix\techreportrv{~\ref{appendix:related-work}}{~C}.

\revheading{R2.D1}: \revitem{The paper repeatedly touts the advantages of multi-objective optimization and emphasizes its soundness. Reduce some of that redundancy and reword the misleading soundness claim. Single-objective optimization is also sound.
} 

We modified the text in the introduction to clarify that multi-objective optimization is a theoretically sound approach to adapting between cost and performance. We removed other mentions in the rest of the paper.


\revheading{R2.D2} \revitem{ It is not clear why optimization time cannot exceed a few seconds. If a stage takes minutes, wouldn't potentially saving 5 minutes be worth investing more than 2 seconds for optimization? In general, where is the point of diminishing returns when investing more into optimization barely improves the objectives?:
}

% \chenghao{
%     \begin{enumerate}
%         \item improve the compile-time searching to support more dense sampling
%         \item The adaptive search strategy is proposed to balance the latency gain and solving time. (R1.D5)
%     \end{enumerate}
% }

We set the solving time to be on the same scale (sub-seconds to seconds) as the VM/Container startup time in the cloud as pointed out by \cite{SharmaCST16,AgarwalJP15,LyuFSSD22}. This is also consistent with our prior experience in solving the resource optimization problem for AliCloud's serverless computing~\cite{LyuFSSD22}.

That said, we agree with the reviewer on the comment. To better balance the effectiveness of optimization and fast solving time, we introduced two techniques in our revision: 
\begin{enumerate}
	\item We improved our compile-time optimization with multi-query plan search, as described in Section~\ref{subsec:multi-pqp-search}. This technique is shown to provide additional performance improvements for several long-running queries with complex query structures. As we use parallel computing for this extension, it does not add to the increase in wall clock time. 
	\item To balance query execution time and solving time, our revision further introduced a (simple) runtime adaptive scheme to adjust the sampling budget based on the predicted latency. This technique is introduced at the end of Section~\ref{subsec:subq-tuning} and used in our new end-to-end experiments in Section 6.3. More specifically, we conducted hyperparameter tuning to derive low, medium, and high values for the sampling budget. Our profiling results show that if the predicted latency using the default configuration is over 10s, it is better to use the median sampling rate; otherwise, we use a low sampling rate. Increasing the sampling rate further does not improve the performance but adds the time cost. This is likely due to the model inaccuracies, which we plan to improve in future work.  

\end{enumerate}


%Our analyses in \rv{\techreport{Appendix~\ref{appendix:adaptive-grid-search}}} show that further increasing the sampling rate does not improve performance but increases solving time, hence negatively impacting query performance.


%To respond the reviewer's request, we proposed a runtime adaptive scheme to pick the proper sampling rate in our method based on the query latency prediction over the default configuration.


\revheading{R2.D3} \revitem{Technical details: What type of embedding is used (Section 4.3)? The model architecture is also not clear. Does the choice of model have a major impact on prediction accuracy? If so, then the model discussion needs more details.}

We thank the reviewer for the comment. 
As has been discussed in our previous work~\cite{spark-moo-icde21,LyuFSSD22}, the choice of model is important, and  the graph transformer network (GTN)~\cite{gtn-neurips19} is shown to be an effective  tool to embed query plans with graph structures to a numerical encoding. 
Besides our previous model analyses in~\cite{LyuFSSD22}, we added additional model discussions in Section~\ref{subsec:model-eval}, including 
\underline{Expt3} on the impact of skewness on our models and \underline{Expt4} on the model generalizability to unseen workloads. 

%\chenghao{
%    \begin{enumerate}
%        \item the model structure has been discussed in our previous work~\cite{spark-moo-icde21}. We used a graph transformer network (GTN)~\cite{gtn-neurips19} to embed the query plan.
%        \item As shown in \cite{spark-moo-icde21}, our GTN-based model outperforms SOTA models in terms of prediction accuracy in the big data analytics systems with a multi-channel input framework to cover features of heterogeneous data structures.
%    \end{enumerate}
%}


\revheading{R2.D4} \revitem{Both random sampling and grid search for parameter value candidates suffer from the curse of dimensionality. Give some more intuition how the crossover approach could address it.}

We significantly extended our paper, including new techniques and new writing, to address the dimensionality of the parameter space. 
%Our changes include the following.
\begin{enumerate}
%\item Initial feature selection: We first clarify that Spark has over 100 parameters and we selected 19 features as follows. (a) We keep query plan parameters $\thetabm_p$ and partition related parameters $\thetabm_s$, which can be replicated to have one copy for each query stage in our fine-grained tuning approach. (b) The dimensionality of the context parameter space ($\thetabm_c$) can reach up to hundreds~\cite{Locat_2022}. To address the issue, we apply the LASSO-path feature selection approach (as in our prior work~\cite{spark-moo-icde21} and in Ottertune~\cite{VanAken:2017:ADM}) and integrate domain knowledge from Spark documentation, resulting in a list of 8 context parameters. More details are in \techreport{Appendix~\ref{appendix:parameter-selection}}.
\item \underline{Feature importance score (FIS) based parameter filtering}: We conducted additional experiments to compute the feature importance scores (FIS) of the 19 parameters in our trained latency and data shuffle models. The FIS of a parameter here is defined to be the increase of the model error if the values of this parameter are randomly shuffled in the training set. Due to space limitations, we include one example in Figure~\ref{fig:rv-fis} in this response document, but leave other plots to 
\techreportrv{Figure~\ref{fig:fi-tpch-lat-all-parameters}-\ref{figs:fi-norm} in Appendix~\ref{appendix:fis-filtering}}{Figure 21-23 in Appendix B.3}. Our main observation is that the FIS values of the parameters, sorted in decreasing order,  follow a long tail distribution. The parameters at the tail, with a cumulative FIS less than 5\% in WMAPE, do not affect the model performance by much and hence can be filtered out. For instance, the threshold of 5\% cumulative FIS means an increment of at most 0.7\% in WMAPE for TPC-H and 1.2\% for TPC-DS in the subQ model.
% Our work applied FIS-based filtering of features, which are the features ranked at the long tail of the distribution with the cumulative loss not exceeding 5\% in WMAPE. 
% Given our current WMAPE results, the exceeding 5\% means 0.7\% more WMAPE in TPC-H and 1.2\% more WMAPE in TPC-DS for the subQ model.
\item \underline{Sampling with FIS-based parameter filtering}: Then we introduced three sampling methods that could leverage FIS-based selection: (a) random sampling with or without parameter filtering; (b) Latin hypercube sampling with or without parameter filtering; (c) adaptive grid search with inherent parameter filtering, as we described in the new paragraph starting with "Sampling methods" on Page 8, which is the last paragraph of Section~\ref{subsec:subq-tuning}.
\item \underline{New experimental results}: We added new results in Figure 11(b)-(c) to show performance metrics (hypervolume and solving time) of the above three sampling methods with parameter filtering. Among them, we report the adaptive grid search to be an overall winner, achieving the highest hypervolume among all FIS-based methods while keeping the solving time under 2s for most queries tested.
%\item \underline{Adaptive sampling}: We also conducted hyperparameter tuning of the sampling budget and further introduce a scheme that adjusts the sampling budget for the adaptive grid search method: If the predicted latency in default configuration is over 10s, we use the median sampling rate; otherwise, a low sampling rate, as introduced in \rv{Section~\ref{subsec:subq-tuning}}. Our analyses in \rv{\techreport{Appendix~\ref{appendix:adaptive-grid-search}}} show that further increasing the sampling rate does not improve performance but increases solving time, hence negatively impacting query performance.
% We provide the low, median, and high sampling rates for the adaptive grid search. When the predicted query latency  The sampling rate will   based on the predicted latency. We report the results in \todo{Table 6}.
% \item \todo{We further introduce the runtime adaptive scheme for the adaptive grid search. When the predicted latency is <10s, we use lower sampling rate, and medium sampling rate if over 10s. The High rate..., added after 2,3 in the paper.} \chenghao{descriptions in Sec5, and experiments in the tables, and report the numbers here: with the adaptiving scheme, we further improvement our performance.} 
% \item Re-organize
\end{enumerate}


% See the points in R1.D4. 

% In addition, add the comment on crossover for R2.D4.


%%%%%%%%%%%% figures in R2.D4 (HV and time)
%\begin{figure*}[t]
%	\centering
%	\setlength{\belowcaptionskip}{0pt}  
%	\setlength{\abovecaptionskip}{0pt}  
%	\begin{tabular}{ccc}
%		\subfigure[\small{{Hypervolume}}]
%        {\label{fig:hv_w_wo_crossover_adaptive_grid}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/adaptive_grid_w_wo_new_theta_c/HV.pdf}}
%		&
%		\subfigure[\small{{Hypervolume}}]
%        {\label{fig:hv_w_wo_crossover_lhs}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/lhs_w_wo_crossover/HV.pdf}}
%		&	
%		\subfigure[\small{{Hypervolume}}]
%        {\label{fig:hv_w_wo_crossover_random}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/random_w_wo_crossover/HV.pdf}}
%		\\
%		\subfigure[\small{{Solving time}}]
%        {\label{fig:time_w_wo_crossover_adaptive_grid}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/adaptive_grid_w_wo_new_theta_c/Time.pdf}}
%		&
%		\subfigure[\small{{Solving time}}]
%        {\label{fig:time_w_wo_crossover_lhs}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/lhs_w_wo_crossover/Time.pdf}}
%		&	
%		\subfigure[\small{{Solving time}}]
%        {\label{fig:time_w_wo_crossover_random}\includegraphics[width=.24\linewidth]{figs/appendix_expt_compile_time_opt/random_w_wo_crossover/Time.pdf}}
%	\end{tabular}
%	\caption{\small{{Comparison of Hypervolume and solving time with/without new $\bm{\theta_c}$ extension for three sampling methods}}}
%	\label{figs:comp_hv_time_w_wo_new_theta_c_all_sampling}
%	\vspace{-0.1in}
%\end{figure*}

%%%%%%%%%%% figures in R2.D4 (Pareto frontiers)
%\begin{figure*}[t]
%	\centering
%	\setlength{\belowcaptionskip}{0pt}  
%	\setlength{\abovecaptionskip}{0pt}  
%	\begin{tabular}{lccc}
%		\subfigure[\small{{TPCH-Q1 with LHS}}]
%        {\label{fig:pareto_tpch_q1}\includegraphics[width=.23\linewidth]{figs/appendix_expt_compile_time_opt/lhs_w_wo_crossover/TPCH/query_1-1_n_3.pdf}}
%        &
%        \subfigure[\small{{TPCDS-Q78 with LHS}}]
%        {\label{fig:pareto_tpcds_q32}\includegraphics[width=.23\linewidth]{figs/appendix_expt_compile_time_opt/lhs_w_wo_crossover/TPCDS/query_78-1_n_11.pdf}}
%        &
%        \subfigure[\small{{TPCH-Q1 with random sampling}}]
%        {\label{fig:pareto_tpch_q1}\includegraphics[width=.23\linewidth]{figs/appendix_expt_compile_time_opt/random_w_wo_crossover/TPCH/query_1-1_n_3.pdf}}
%        &		
%		\subfigure[\small{{TPCDS-Q13 with random sampling}}]
%        {\label{fig:pareto_tpcds_q13}\includegraphics[width=.23\linewidth]{figs/appendix_expt_compile_time_opt/random_w_wo_crossover/TPCDS/query_13-1_n_7.pdf}}		
%	\end{tabular}
%	\caption{\small{{Comparison of Pareto frontiers with/without crossover in LHS and random-sampling}}}
%	\label{figs:comp_pareto_w_wo_crossover_lhs_random}
%	\vspace{-0.1in}
%\end{figure*}

We further clarify that the crossover approach is used in the step to enrich the $\thetabm_c$ candidates in order to address the missing Pareto solutions. Crossover is a genetic operation that tends to inherit promising regions of parameters from the promising candidates, and generate new candidates to potentially improve the performance, without searching the high-dimensional space. Our profiling results show that this technique helps find more global Pareto optimal solutions, especially, in the middle region of the Pareto front. More analyses are in \techreportrv{Appendix \ref{appendix:more-expt-sampling}}{Appendix B.9}.  

%\qi{
%%1. overall new theta\_c extension helps. crossover is one option.
%%2. verify with adaptive grid.
%\underline{How new $\bm{\theta_c}$ extension helps?}
%The procedure of new $\bm{\theta_c}$ extension helps find more global Pareto optimal solutions, where crossover is one option used along with LHS or random-sampling.
%Crossover is a genetic operation that tends to inherit promising regions of parameters from the promising candidates, and generate new candidates to potentially improve the performance, without searching the high-dimensional space.
%Another option used in adaptive grid-search is random-sampling as crossover cannot generate new $\bm{\theta_c}$.
%Figures \ref{figs:comp_hv_time_w_wo_new_theta_c_all_sampling} in Appendix \ref{appendix:more-expt-sampling} verify that all options of new $\bm{\theta_c}$ extension work to find global Pareto optimal solutions by improving HV. 
%And crossover helps to find better global Pareto optimal solutions in the middle region of objective space (shown in Figures  \ref{figs:comp_pareto_w_wo_crossover_lhs_random}). 
%More analysis can be found in Appendix \ref{appendix:more-expt-sampling}.
%}


\revheading{R2.D5} \revitem{Proposition 5.1 seems obvious, if subqueries are treated as independent. Does it still hold when taking their interactions into account (W2, W3)?}

We clarify that Proposition \ref{prop:need_opt_p} is for compile-time optimization, where indeed we made simplifying assumptions to enable efficient algorithms. In particular, it assumes that for a specific $\bm{\theta_c}$, the subquery structure is fixed and $\bm{\theta_p}$ can be  set for different subqueries independently. The rationale of these assumptions is to recommend a good $\bm{\theta_c}$ by considering the correlation with $\bm{\theta_p}$ while achieving high computational efficiency.

In the revision, we introduced a compile-time technique that samples multiple physical plans for each query, as described in Section~\ref{subsec:multi-pqp-search}. Then our runtime optimization further relaxes the assumptions by continuing to adjust the parameters and physical plans as runtime statistics are collected from the completed stages. 

%Proposition \ref{prop:need_opt_p} is for compile-time optimization, where indeed we made an assumption to simply the optimization problem.
%Under this assumption, for a specific $\bm{\theta_c}$, sub-query structures remain unchanged during compile-time optimization and $\bm{\theta_p}$ are set for sub-queries independently.
%The rational of this assumption is to recommend optimal and reasonable $\bm{\theta_c}$ by considering correlation of $\bm{\theta_p}$ while with high computational efficiency.
%Runtime optimization addresses this assumption by introducing Pareto sets from multiple LQP structures in compile-time optimization and changing sub-query plans with accurate statistics at runtime, which maintains high efficiency while considering multiple LQP structures.
  

\revheading{R2.D6:} \revitem{The discussion how some initial choice of join algorithm limits options for later reoptimization (Section 5.2) needs to be broadened. Does it only apply to this specific scenario? Or are there other limitations like it in Spark?}

To respond to the reviewer's question, we added concrete examples in Section~\ref{sec:runtime-opt} to illustrate why setting join threshold values either too high or too low will lead to suboptimal query plans. 
It does only apply to this specific scenario due to design decisions made by Spark committers, and so far we have not found other similar limitations in Spark.
% \chenghao{\begin{enumerate}
%     \item Clarify the limitation of the join algorithm transformation in Spark. 
%     \item Clarify this is the only restriction appeared in the default Spark AQE rules that affects our optimization.
% \end{enumerate}
% }


==> response/R4.tex <==
\section*{Reviewer 4}

All of our references to the appendices refer to our tech report online: 
https://chenghao.pages.dev/papers/vldb24-lyu-tr.pdf~\cite{tech-report}

\revheading{R4.D1:} \revitem{In the experiments, the paper says: "To collect training data, we further treat these queries as templates to generate 50k distinct parameterized queries for TPC-H and TPC-DS, respectively". Thus, it seems that queries are following the same patterns as they use the same template. However, this may not be true in practice where new query workloads may be different from the training workloads. Thus, I would like to see how the proposed approach work on different workloads with different query patterns.}

We thank the reviewer for this suggestion. To investigate the generalizability of our learned models to unseen workloads, 
%To address concerns about the generalization of our approach to different workloads with varying query patterns, 
we conducted a new experiment, \underline{Expt 4} in Section 6.1. We investigated two approaches.
\begin{enumerate}
    \item \textit{Direct Application}: The first approach applies the latency model trained on TPC-DS directly to TPC-H, or vice versa. However, it leads to high errors due to significant differences in the running environments. 
    \item \textit{Graph Embedding Transfer}: Our second approach transfers the graph embedding through the GTN model and retrains only the regressor for latency prediction, which is relatively fast. Our results indicate that graph embeddings trained on a workload with a broader range of query operators (e.g., TPC-DS) can be transferred effectively, resulting in a modest 0.06 WMAPE increase for the subQ model and a 0.06 and 0.16 WMAPE decrease for QS and \collap\ models, respectively. 
\end{enumerate}
Due to space constraints, we summarized the most significant results in the main paper.  Detailed numbers of all our trained models can be found in \techreportrv{Appendix~\ref{appendix:more-generalization}}{Appendix B.7}. Overall, the results of this new experiment improved our paper with positive evidence on the transfer learning ability of the GTN model, which is the most expensive part of model training. 
%We further explore the generalizability of our trained model to unseen workloads. The first approach applies the latency model trained on TPC-DS directly to TPC-H, or vice versa. However, it leads to high errors due to significant differences in the running environments. The second approach transfers the graph embedding through the GTN model and retrains only the regressor for latency prediction, which is relatively fast. Our results indicate that graph embeddings trained on a workload with a broader range of query operators (e.g., TPC-DS) can be transferred effectively, resulting in a modest 0.06 WMAPE increase for the subQ model and a 0.06 and 0.16 WMAPE decrease for QS and \collap, respectively. More details can be found in \techreport{Appendix~\ref{appendix:more-generalization}}.

\revheading{R4.D2:} \revitem{It would be interesting to discuss whether or how to extend the proposed approach to other databases or data systems.}

Our work has the potential to apply to other systems that can observe runtime statistics and have the runtime adaptability. These systems include Presto~\cite{Presto}, Greenplum Database~\cite{Greenplum}, Microsoft SQL Server~\cite{Microsoft2021}, MaxCompute~\cite{maxcompute}, etc. However, the exact runtime statistics may vary across these systems: a system with richer statistics allows precise models to be trained which in turn enables effective optimization, whereas a system with limited statistics will experience suboptimal results. 
Therefore, it will be an interesting study in our future work to extend our approach to some of these systems. We have included this discussion in the conclusions and future work section. %to reflect this potential direction.

% It is possible to extend our proposed approach to other databases or big data analytics systems if there are (1) clear performance objectives, (2) queries formalized in topological graph that can be partitioned into different stages connected by dependencies, (3) the adaptive execution scheme with tunable parameters for the remaining computational tasks.
% However, applying to a new system will include a bunch of engineering efforts to cover the runtime feature exposure, trace collection, feature extraction, and model training/tuning. 
% \todo{CH: add to appendix?}
